Conjunctive Query Answering for the Description Logic SHIQ

Conjunctive queries play an important role as an expressive query language for Description Logics (DLs). Although modern DLs usually provide for transitive roles, conjunctive query answering over DL knowledge bases is only poorly understood if transitive roles are admitted in the query. In this paper, we consider unions of conjunctive queries over knowledge bases formulated in the prominent DL SHIQ and allow transitive roles in both the query and the knowledge base. We show decidability of query answering in this setting and establish two tight complexity bounds: regarding combined complexity, we prove that there is a deterministic algorithm for query answering that needs time single exponential in the size of the KB and double exponential in the size of the query, which is optimal. Regarding data complexity, we prove containment in co-NP.

==> conclusions.tex <==
\section{Conclusions}\label{sect:conclusions}

With the decision procedure presented for entailment of unions of 
conjunctive queries in \SHIQ, we close a long standing open problem. The 
solution has immediate consequences on related areas, as it shows that 
several other open problems such as query answering, query containment 
and the extension of a knowledge base with weakly safe Datalog rules for 
\SHIQ are decidable as well. Regarding combined complexity, we present a 
deterministic algorithm that needs time single exponential in the size 
of the KB and double exponential in the size of the query, which gives a 
tight upper bound for the problem. This result shows that deciding 
conjunctive query entailment is strictly harder than instance checking 
for \SHIQ. We further prove co-\NPclass-completeness for data 
complexity. Interestingly, this shows that regarding data complexity 
deciding UCQ entailment is (at least theoretically) not harder than 
instance checking for \SHIQ, which was also a previously open question. 

It will be part of our future work to extend this procedure to \SHOIQ, 
which is the DL underlying OWL DL. We will also attempt to find more 
implementable algorithms for query answering in \SHIQ. Carrying out the 
query rewriting steps in a more goal directed way will be crucial to 
achieving this. 


==> decisionprocedure.tex <==
\section{The Decision Procedure}
\label{sect:decisionprocedure}

We now devise a decision procedure for entailment of unions of Boolean 
conjunctive queries that uses, for each disjunct, the queries obtained 
in the rewriting process as defined in the previous section. Detailed 
proofs for the lemmas and theorems in this section can again be found in 
the appendix. For a knowledge base \KB and a union of Boolean 
conjunctive queries $\Q_1 \vee \ldots \vee \Q_\ell$, we show how we can 
use the queries in $\trees{\Q_i}$ and $\groundings{\Q_i}$ for $1 
\leq i \leq \ell$ in order to build a set of knowledge bases 
$\KB_1, \dots, \KB_n$ such that $\KB \models \Q_1 \vee \ldots \vee 
\Q_\ell$ iff all the $\KB_i$ are inconsistent. This gives rise to two 
decision procedures: a deterministic one in which we enumerate all 
$\KB_i$, and which we use to derive a tight upper bound for the combined 
complexity; and a non-deterministic one in which we guess a $\KB_i$, and 
which yields a tight upper bound for the data complexity. Recall that, 
for combined complexity, the knowledge base \KB and the queries $\Q_i$ 
both count as input, whereas for the data complexity only the ABox \AB 
counts as an input, and all other parts are assumed to be fixed. 



\subsection{A Deterministic Decision Procedure for Query Entailment in 
\SHIQ}\label{sect:deterministic}

We first define the deterministic version of the decision procedure and 
give an upper bound for its combined complexity. The given algorithm 
takes as input a union of connected conjunctive queries and works under 
the unique name assumption (UNA). We show afterwards how it can be 
extended to an algorithm that does not make the UNA and that takes 
arbitrary UCQs as input, and that the complexity results carry over. 

We construct a set of knowledge bases that extend the original knowledge 
base \KB both w.r.t.\ the TBox and ABox. The extended knowledge bases 
are such that a given KB \KB entails a query \Q iff all the extended KBs 
are inconsistent. We handle the concepts obtained from the tree-shaped 
queries differently to the ground queries: the axioms we add to the TBox 
prevent matches for the tree-shaped queries, whereas the extended ABoxes 
contain assertions that prevent matches for the ground queries. 

\begin{definition}
  Let \KBDef be a \SHIQ knowledge base and $\Q = \Q_1 \vee \ldots \vee 
  \Q_\ell$ a union of Boolean conjunctive queries. We set  
  \begin{enumerate}
    \item
      $T := \trees{\Q_1} \cup \ldots \cup \trees{\Q_\ell}$,
    \item 
      $G := \groundings{\Q_1} \cup \ldots \cup \groundings{\Q_\ell}$, 
      and 
    \item\label{it:treeGCIs} 
      $\TB_\Q := \{\top \sqsubseteq \neg C \mid C(v) \in T\}$.
  \end{enumerate}
  An \emph{extended knowledge base} $\KB_\Q$ w.r.t.\ \KB and \Q is a 
  tuple $(\TB \cup \TB_\Q, \RB, \AB \cup \AB_\Q)$ such that $\AB_\Q$ 
  contains, for each $\Q' \in G$, at least one assertion $\neg at$ with 
  $at \in \Q'$. 
  %$\AB_\Q \in \{\{\neg at_1, \ldots, \neg at_n\} \mid at_i \in \Q'_i 
  %\mbox{ and } \{\Q'_1, \ldots, \Q'_n\} = G\}$.
\end{definition}

Informally, the extended TBox $\TB \cup \TB_\Q$ ensures that there are 
no tree matches. Each extended ABox $\AB \cup \AB_\Q$ contains, for each 
ground query $\Q'$ obtained in the rewriting process, at least one 
assertion $\neg at$ with $at \in \Q'$ that ``spoils'' a match for $\Q'$. 
A model for such an extended ABox can, therefore, not satisfy any of the 
ground queries. If there is a model for any of the extended knowledge 
bases, we know that this is a counter-model for the original query.

We can now use the extended knowledge bases in order to define the 
deterministic version of our algorithm for deciding entailment of unions 
of Boolean conjunctive queries in \SHIQ. 

\begin{definition}\label{def:algodeterministic}
  Given a \SHIQ knowledge base \KBDef and a union of connected Boolean 
  conjunctive queries \Q as input, the algorithm answers ``\KB entails 
  \Q'' if each extended knowledge base w.r.t.\ \KB and \Q is 
  inconsistent and it answers ``\KB does not entail \Q'' otherwise.
\end{definition}

The following lemma shows that the above described algorithm is indeed 
correct. 

\begin{lemma}\label{lem:correctness}
  Let \KB be a \SHIQ knowledge base and \Q a union of connected Boolean 
  conjunctive queries. Given \KB and \Q as input, the algorithm from 
  Definition~\ref{def:algodeterministic} answers ``\KB entails \Q'' iff 
  $\KB \models \Q$ under the unique name assumption.
\end{lemma}

% if: \KB \models \Q -> answers \KB entails \Q
% only if: answers \KB entails \Q -> \KB \models \Q
% or cp: \KB \not\models \Q -> answers \KB does not entails \Q
In the proof of the if direction for the above lemma, we can use a 
canonical model \I of \KB in order to guide the rewriting process. For 
the only if direction, we assume to the contrary of what is to be shown 
that there is no consistent extended knowledge base, but $\KB 
\not\models \Q$. We then use a model \I of \KB such that $\I 
\not\models \Q$, which exists by assumption, and show that \I is also a 
model of some extended knowledge base. 



\subsubsection{Combined Complexity of Query Entailment in \SHIQ}
\label{sect:combinedcomplexity}

According to the above lemma, the algorithm given in 
Definition~\ref{def:algodeterministic} is correct. We now analyse its 
combined complexity and thereby prove that it is also terminating. 

For the complexity analysis, we assume, as usual 
\cite{HuMS05a,CGLL06a,OrCE06a}, that all concepts in concept atoms and 
ABox assertions are literals, i.e., concept names or negated concept 
names. If the input query or ABox contains non-literal atoms or 
assertions, we can easily transform these into literal ones in a truth 
preserving way: for each concept atom $C(t)$ in the query where $C$ is a 
non-literal concept, we introduce a new atomic concept $A_C \in \NC$, 
add the axiom $C \sqsubseteq A_C$ to the TBox, and replace $C(t)$ with 
$A_C(t)$; for each non-literal concept assertion $C(a)$ in the ABox, we 
introduce a new atomic concept $A_C \in \NC$, add an axiom $A_C 
\sqsubseteq C$ to the TBox, and replace $C(a)$ with $A_C(a)$. Such a 
transformation is obviously polynomial, so without loss of generality, 
it is safe to assume that the ABox and query contain only literal 
concepts. This has the advantage that the size of each atom and ABox 
assertion is constant. 

Since our algorithm involves checking the consistency of a \SHIQR 
knowledge base, we analyse the complexity of this reasoning 
service.~\citeA{Tobi01a} shows an \ExpTime upper bound for deciding the 
consistency of \SHIQ knowledge bases (even with binary coding of 
numbers) by translating a \SHIQ KB to an equisatisfiable \ALCQIb 
knowledge base. The $b$ stands for \emph{safe Boolean role expressions} 
built from \ALCQIb roles using the operator $\sqcap$ (role 
intersection), $\sqcup$ (role union), and $\neg$ (role 
negation/complement) such that, when transformed into disjunctive normal 
form, every disjunct contains at least one non-negated conjunct. Given a 
query \Q and a \SHIQ knowledge base $\KBDef$, we reduce query entailment 
to deciding knowledge base consistency of an extended \SHIQR knowledge 
base $\KB_\Q = (\TB \cup \TB_\Q, \RB, \AB \cup \AB_\Q)$. Recall that 
$\TB_\Q$ and $\AB_\Q$ are the only parts that contain role conjunctions 
and that we use role negation only in ABox assertions. We extend the 
translation given for \SHIQ so that it can be used for deciding the 
consistency of \SHIQR KBs. Although the translation works for all \SHIQR 
KBs, we assume the input KB to be of exactly the form of extended 
knowledge bases as described above. This is so because the translation 
for unrestricted \SHIQR is no longer polynomial, as in the case of 
\SHIQ, but exponential in the size of the longest role conjunction under 
a universal quantifier. Since role conjunctions occur only in the 
extended ABox and TBox, and since the size of each role conjunction is, 
by Lemma~\ref{lem:counting}, polynomial in the size of \Q, the 
translation is only exponential in the size of the query in the case of 
extended knowledge bases. 

We assume here, as usual, that all concepts are in \emph{negation normal 
form (NNF)}; any concept can be transformed in linear time into an 
equivalent one in NNF by pushing negation inwards, making use of de 
Morgan's laws and the duality between existential and universal 
restrictions, and between atmost and atleast number restrictions 
($\leqslant n\; r.C$ and $\geqslant n\; r.C$ respectively) 
\cite{HoST00a}. For a concept $C$, we use $\dot\neg C$ to denote the NNF 
of $\neg C$. 

We define the \emph{closure} $\cl{C, \RB}$ of a concept $C$ w.r.t.\ a 
role hierarchy \RB as the smallest set satisfying the following 
conditions:
\begin{itemize}
  \item 
    if $D$ is a sub-concept of $C$, then $D \in \cl{C, \RB}$,
  \item 
    if $D \in \cl{C, \RB}$, then $\dot\neg D \in \cl{C, \RB}$,
  \item 
    if $\forall r.D \in \cl{C, \RB}, s \sssR r$, and $s \in \transR$, 
    then $\forall s.D \in \cl{C, \RB}$.
\end{itemize}

We now show how we can extend the translation from \SHIQ to \ALCQIb 
given by Tobies. We first consider $\SHIQR$-concepts and then extend the 
translation to KBs. 

\begin{definition}
  For a role hierarchy \RB and roles $r, r_1, \ldots, r_n$, let 
  $$
    \up{r} = \bigsqcap \limits_{r \ssssR s} s \mbox{\hspace{.4cm} and 
    \hspace{.4cm}}\up{r_1 \sqcap \ldots \sqcap r_n} = \up{r_1} \sqcap 
    \ldots \sqcap \up{r_n}.
  $$
  \mathdefend
\end{definition}

Please note that, since $r \sssR r$, $r$ occurs in \up{r}.\hfill{}

\begin{lemma}\label{lem:uparrow}
  Let \RB be a role hierarchy, and $r_1, \ldots, r_n$ roles. For 
  every interpretation \I such that $\I \models \RB$, it holds that 
  $\Int{(\up{r_1 \sqcap \ldots \sqcap r_n})} = \Int{(r_1 \sqcap \ldots 
  \sqcap r_n)}$.
\end{lemma}

With the extended definition of $\uparrow$ on role conjunctions, we can 
now adapt the definition (Def.\ 6.22) that Tobies provides for 
translating $\SHIQ$-concepts into $\ALCQIb$-concepts.

\begin{definition}\label{def:translation}
  Let $C$ be a $\SHIQR$-concept in NNF and \RB a role hierarchy. For 
  every concept $\forall (r_1 \sqcap \ldots \sqcap r_n).D \in 
  \cl{C, \RB}$, let $X_{r_1 \sqcap \ldots \sqcap r_n, D} \in \NC$ be a 
  unique concept name that does not occur in $\cl{C, \RB}$. Given a role 
  hierarchy \RB, we define the function $\mn{tr}$ inductively on the 
  structure of concepts by setting
  $$
  \begin{array}{rcl}
    \tr{A} & = & A \mbox{ for all A } \in \NC\\
    \tr{\neg A} & = & \neg A \mbox{ for all A } \in \NC\\
    \tr{C_1 \sqcap C_2} & = & \tr{C_1} \sqcap \tr{C_2}\\
    \tr{C_1 \sqcup C_2} & = & \tr{C_1} \sqcup \tr{C_2}\\
    \tr{\bowtie n (r_1 \sqcap \ldots \sqcap r_n).D} & = & (\bowtie 
    n \up{r_1 \sqcap \ldots \sqcap r_n}.\tr{D})\\
    \tr{\forall (r_1 \sqcap \ldots \sqcap r_n).D} & = & X_{r_1 
    \sqcap \ldots \sqcap r_n, D}\\
    \tr{\exists (r_1 \sqcap \ldots \sqcap r_n).D} & = & \neg 
    (X_{r_1 \sqcap \ldots \sqcap r_n, \dot \neg D})\\
  \end{array}
  $$
  where $\bowtie$ stands for $\leqslant$ or $\geqslant$. Set 
  $\mn{tc}((r_1 \sqcap \ldots \sqcap r_n), \RB) := \{(t_1 \sqcap \ldots 
  \sqcap t_n) \mid t_i \sssR r_i \mbox{ and } t_i \in \transR$ for each 
  $i$ such that $1 \leq i \leq n\}$ and define an extended 
  TBox $\TB_{C, \RB}$ as 
  $$
  {\setlength{\arraycolsep}{0em}
  \begin{array}{rcll}
    \TB_{C, \RB} & = & \{ X_{r_1 \sqcap \ldots \sqcap r_n, D} \equiv 
    \forall \up{r_1 \sqcap \ldots \sqcap r_n}.\tr{D} & \mid \forall 
    (r_1 \sqcap \ldots \sqcap r_n).D \in \mn{cl}(C, \RB)\}\mbox{ }\cup\\
%    & & & \forall \up{r_1 \sqcap \ldots \sqcap r_n}.\tr{D} \mid \forall 
%    (r_1 \sqcap \ldots \sqcap r_n).D \in \mn{cl}(C, \RB)\}\mbox{ }\cup\\
%    & & \{ & X_{r_1 \sqcap \ldots \sqcap r_n, D} \sqsubseteq \bigsqcap 
%    \limits_{T \in \mn{tc}(r_1 \sqcap \ldots \sqcap r_n, \RB)} \forall 
%    \up{T}.X_{T, D}\}\\
    & & \{ X_{r_1 \sqcap \ldots \sqcap r_n, D} \sqsubseteq \forall 
    \up{T}.X_{T, D} & \mid T \in \mn{tc}(r_1 \sqcap \ldots \sqcap r_n, 
    \RB)\}\\
  \end{array}
  }
  $$
  \mathdefend
\end{definition}

\begin{lemma}\label{lem:tr}
  Let $C$ be a $\SHIQR$-concept in NNF, \RB a role hierarchy, and 
  $\mn{tr}$ and $\TB_{C, \RB}$ as defined in 
  Definition~\ref{def:translation}. The concept $C$ is satisfiable 
  w.r.t.\ \RB iff the \ALCQIb-concept $\tr{C}$ is satisfiable w.r.t.\ 
  $\TB_{C, \RB}$.
\end{lemma}

Given Lemma~\ref{lem:uparrow}, the proof of Lemma~\ref{lem:tr} is a 
long, but straightforward extension of the proof given by 
\citeA[Lemma~6.23]{Tobi01a}.

We now analyse the complexity of the above described problem. Let $m := 
|\RB|$ and $r_1 \sqcap \ldots \sqcap r_n$ the longest role conjunction 
occurring in $C$, i.e., the maximal number of roles that occur in a role 
conjunction in $C$ is $n$. The TBox $\TB_{C, \RB}$ can contain 
exponentially many axioms in $n$ since the cardinality of the set 
$\mn{tc}((r_1 \sqcap \ldots \sqcap r_n), \RB)$ for the longest role 
conjunction can only be bounded by $m^n$ because each $r_i$ can have 
more than one transitive sub-role. It is not hard to check that the size 
of each axiom is polynomial in $|C|$. Since deciding whether an \ALCQIb 
concept $C$ is satisfiable w.r.t.\ an \ALCQIb TBox \TB is an 
\ExpTime-complete problem (even with binary coding of numbers) 
\cite[Thm.\ 4.42]{Tobi01a}, the satisfiability of a $\SHIQR$-concept 
$C$ can be checked in time $2^{p(m) 2^{p(n)}}$. 

We now extend the translation from concepts to knowledge bases. Tobies 
assumes that all role assertions in the ABox are of the form $r(a, b)$ 
with $r$ a role name or the inverse of a role name. Extended ABoxes 
contain, however, also negated roles in role assertions, which require a 
different translation. A positive role assertion such as $r(a, b)$ is 
translated in the standard way by closing the role upwards. The only 
difference of using $\uparrow$ directly is that we additionally split 
the conjunction $(\up{r})(a, b) = (r_1 \sqcap \ldots \sqcap r_n)(a, b)$ 
into $n$ different role assertions $r_1(a, b), \ldots, r_n(a, b)$, which 
is clearly justified by the semantics. For negated roles in a role 
assertion such as $\neg r(a, b)$, we close the role downwards instead of 
upwards and add a role atom $\neg s(a, b)$ for each sub-role $s$ of 
$r$. This is again justified by the semantics. Let $\KB = (\TB \cup 
\TB_\Q, \RB, \AB \cup \AB_\Q)$ be an extended knowledge base. More 
precisely, we set 
$$
  \tr{\TB \cup \TB_\Q} := \{\tr{C} \sqsubseteq \tr{D} \mid C \sqsubseteq 
  D \in \TB \cup \TB_\Q\},
$$ 
$$
  \begin{array}{l l}
    \tr{\AB \cup \AB_\Q} := & \{(\tr{C})(a) \mid C(a) \in \AB \cup 
          \AB_\Q\} \mbox{ } \cup \\
      & \{s(a, b) \mid r(a, b) \in \AB \cup \AB_\Q \mbox{ and } r \sssR 
          s\} \mbox{ } \cup \\
      & \{\neg s(a, b) \mid \neg r(a, b) \in \AB \cup \AB_\Q \mbox{ and  
          } s \sssR r\},
  \end{array}
$$
and we use \tr{\KB} to denote the \ALCQIb knowledge base (\tr{\TB \cup 
\TB_\Q}, \tr{\AB \cup \AB_\Q}).

For the complexity of deciding the consistency of a translated \SHIQR 
knowledge base, we can apply the same arguments as above for concept 
satisfiability, which gives the following result: 

\begin{lemma}\label{lem:shiqrconsistency} 
  Given a \SHIQR knowledge base \KBDef where $m := |\KB|$ and the size 
  of the longest role conjunction is $n$, we can decide consistency of 
  \KB in deterministic time $2^{p(m) 2^{p(n)}}$ with $p$ a polynomial.
\end{lemma}

We are now ready to show that the algorithm given in 
Definition~\ref{def:algodeterministic} runs in deterministic time single 
exponential in the size of the input KB and double exponential in the 
size of the input query.

\begin{lemma}\label{lem:combinedcomplexity}
  Let \KBDef be a \SHIQ knowledge base with $m = |\KB|$ and \Q a union 
  of connected Boolean conjunctive queries with $n = |\Q|$. Given \KB 
  and \Q as input, the algorithm given in 
  Definition~\ref{def:algodeterministic} decides whether $\KB \models 
  \Q$ under the unique name assumption in deterministic time in 
  $2^{p(m) 2^{p(n)}}$. 
\end{lemma}

In the proof of the above lemma, we show that there is some polynomial 
$p$ such that we have to check at most $2^{p(m) 2^{p(n)}}$ extended 
knowledge bases for consistency and that each consistency check can be 
done in this time bound as well. 

More precisely, let $\Q = \Q_1 \vee \ldots \vee \Q_\ell, T = 
\trees{\Q_1} \cup \ldots \cup \trees{\Q_\ell}$, and $G = 
\groundings{\Q_1} \cup \ldots \cup \groundings{\Q_\ell}$. Together with 
Lemma~\ref{lem:counting}, we get that $\card{T}$ and $\card{G}$ are 
bounded by $2^{p(n) \cdot \log p(m)}$ for some polynomial $p$ and that 
the size of each query in $G$ and $T$ is polynomial in $n$. Each of the 
$2^{p(n) \cdot \log p(m)}$ ground queries in $G$ contributes at most 
$p(n)$ negated assertion to an extended ABox $\AB_\Q$. Hence, there are 
at most $2^{p(m) 2^{p(n)}}$ extended ABoxes $\AB_\Q$ and, therefore, 
$2^{p(m) 2^{p(n)}}$ extended knowledge bases that have to be tested for 
consistency. 

Given the bounds on the cardinalities of $T$ and $G$ and the fact that 
the size of each query in $T$ and $G$ is polynomial in $n$, it is not 
hard to check that the size of each extended knowledge base $\KB_\Q = 
(\TB \cup \TB_\Q, \RB, \AB \cup \AB_\Q)$ is bounded by $2^{p(n) \cdot 
\log p(m)}$ and that each $\KB_\Q$ can be computed in this time bound as 
well. Since only the extended parts contain role conjunctions and the 
number of roles in a role conjunction is polynomial in $n$, there is a 
polynomial $p$ such that  
\begin{enumerate}
  \item
    $|\tr{\TB}| \leq p(m)$, 
  \item
    $|\tr{\TB_\Q}| \leq 2^{p(n) \cdot \log p(m)}$, 
  \item
    $|\tr{\AB}| \leq p(m)$, 
  \item
    $|\tr{\AB_\Q}| \leq 2^{p(n) \cdot \log p(m)}$, and, hence, 
  \item
    $|\tr{\KB_\Q}| \leq 2^{p(n) \cdot \log p(m)}$.
\end{enumerate}
By Lemma~\ref{lem:shiqrconsistency}, each consistency check can be done 
in time $2^{p(m) 2^{p(n)}}$ for some polynomial $p$. Since we have to 
check at most $2^{p(m) 2^{p(n)}}$ extended knowledge bases for 
consistency, and each check can be done in time $2^{p(m) 2^{p(n)}}$, we 
obtain the desired upper bound. 

We now show that this result carries over even when we do not restrict 
interpretations to the unique name assumption.
  
\begin{definition}
  Let \KBDef be a \SHIQ knowledge base and \Q a \SHIQ union of Boolean 
  conjunctive queries. For a partition \Pmc of \indA, a knowledge base 
  $\KB^\Pmc = (\TB, \RB, \AB^\Pmc)$ and a query $\Q^\Pmc$ are called an 
  \emph{$\AB$-partition w.r.t.\ \KB and \Q} if $\AB^\Pmc$ and $\Q^\Pmc$ 
  are obtained from \AB and \Q as follows:\\
  For each $P \in \Pmc$
  \begin{enumerate}
    \item 
      Choose one individual name $a \in P$.
    \item
      For each $b \in P$, replace each occurrence of $b$ in \AB and \Q 
      with $a$. 
  \end{enumerate}
\end{definition}

Please note that w.l.o.g.\ we assume that all constants that occur in 
the query occur in the ABox as well and that thus a partition of the 
individual names in the ABox also partitions the query.

\begin{lemma}\label{lem:UNA}
  Let \KBDef be a \SHIQ knowledge base and \Q a union of Boolean 
  conjunctive queries. $\KB \not\models \Q$ without making the unique 
  name assumption iff there is an \AB-partition $\KB^\Pmc = (\TB, \RB, 
  \AB^\Pmc)$ and $\Q^\Pmc$ w.r.t.\ \KB and \Q such that $\KB^\Pmc 
  \not\models \Q^\Pmc$ under the unique name assumption.
\end{lemma}

Let \KBDef be a knowledge base in a Description Logic $\mathcal{DL}$, 
\Cmc be the complexity class such that deciding whether $\KB \models \Q$ 
under the unique name assumption is in \Cmc, and let $n = 2^{|\AB|}$. 
Since the number of partitions for an ABox is at most exponential in the 
number of individual names that occur in the ABox, the following is a 
straightforward consequence of the above lemma: for a Boolean 
conjunctive $\mathcal{DL}$ query \Q, deciding whether $\KB \models \Q$ 
without making the unique name assumption can be reduced to deciding $n$ 
times a problem in \Cmc. 

In order to extend our algorithm to unions of possibly unconnected 
Boolean conjunctive queries, we first transform the input query \Q into 
conjunctive normal form (CNF). We then check entailment for each 
conjunct $\Q_i$, which is now a union of connected Boolean conjunctive 
queries. The algorithm returns ``\KB entails \Q'' if each entailment 
check succeeds and it answers ``\KB does not entail \Q'' otherwise. By 
Lemma~\ref{lem:cnf} and Lemma~\ref{lem:correctness}, the algorithm is 
correct. 

Let \KB be a knowledge base in a Description Logic $\mathcal{DL}$, \Q a 
union of connected Boolean conjunctive $\mathcal{DL}$ queries, and \Cmc 
the complexity class such that deciding whether $\KB \models \Q$ is in 
\Cmc. Let $\Q'$ be a union of possibly unconnected Boolean conjunctive 
queries and $\mn{cnf}(\Q')$ the CNF of $\Q'$. Since the number of 
conjuncts in $\mn{cnf}(\Q')$ is at most exponential in $|\Q'|$, deciding 
whether $\KB \models \Q'$ can be reduced to deciding $n$ times a problem 
in \Cmc, with $n = 2^{p(|\Q'|)}$ and $p$ a polynomial. 

The above observation together with the results from 
Lemma~\ref{lem:combinedcomplexity} gives the following general result:

\begin{theorem}\label{thm:combinedcomplexity}
  Let \KBDef be a \SHIQ knowledge base with $m = |\KB|$ and $\Q$ a union 
  of Boolean conjunctive queries with $n = |\Q|$. Deciding whether $\KB 
  \models \Q$ can be done in deterministic time in $2^{p(m) 2^{p(n)}}$. 
\end{theorem}

A corresponding lower bound follows from the work by \citeA{Lutz07a}. 
Hence the above result is tight. The result improves the known 
co-3\NExpTime upper bound for the setting where the roles in the query 
are restricted to simple ones \cite{OrCE06b}. 

\begin{corollary}
  Let \KB be a \SHIQ knowledge base with $m = |\KB|$ and \Q a union of 
  Boolean conjunctive queries with $n = |\Q|$. Deciding whether $\KB 
  \models \Q$ is a 2\ExpTime-complete problem. 
\end{corollary}

Regarding query answering, we refer back to the end of 
Section~\ref{pre:sect:cqs}, where we explain that deciding which 
tuples belong to the set of answers can be checked with at most 
$m_\AB^k$ entailment tests, where $k$ is the number of answer 
variables in the query and $m_\AB$ is the number of individual names in 
\indA. Hence, at least theoretically, this is absorbed by the combined 
complexity of query entailment in \SHIQ.


\subsection{A Non-Deterministic Decision Procedure for Query Entailment 
in \SHIQ}\label{sect:nondeterministic}

In order to study the data complexity of query entailment, we devise a 
non-deterministic decision procedure which provides a tight bound for 
the complexity of the problem. Actually, the devised algorithm decides 
non-entailment of queries: we guess an extended knowledge base 
$\KB_\Q$, check whether it is consistent, and return ``\KB does not 
entail \Q'' if the check succeeds and ``\KB entails \Q'' otherwise. 

\begin{definition}\label{def:algonondeterministic}
  Let \TB be a \SHIQ TBox, \RB a \SHIQ role hierarchy, and \Q a union of 
  Boolean conjunctive queries. Given a \SHIQ ABox \AB as input, the 
  algorithm guesses an \AB-partition $\KB^\Pmc = (\TB, \RB, \AB^\Pmc)$ 
  and $\Q^\Pmc$ w.r.t.\ \KB = (\TB, \RB, \AB) and \Q. The query 
  $\Q^\Pmc$ is then transformed into CNF and one of the resulting 
  conjuncts, say $\Q_i^\Pmc$, is chosen. The algorithm then guesses an 
  extended knowledge base $\KB_{\Q_i}^\Pmc = (\TB \cup \TB_{\Q_i}, \RB, 
  \AB^\Pmc \cup \AB^\Pmc_{\Q_i})$ w.r.t.\ $\KB^\Pmc$ and $\Q_i^\Pmc$ and 
  returns ``\KB does not entail \Q'' if $\KB_{\Q_i}^\Pmc$ is consistent 
  and it returns ``\KB entails \Q'' otherwise.
\end{definition}

Compared to the deterministic version of the algorithm given in 
Definition~\ref{def:algodeterministic}, we do not make the UNA but guess 
a partition of the individual names. We also non-deterministically 
choose one of the conjuncts that result from the transformation into 
CNF. For this conjunct, we guess an extended ABox and check whether the 
extended knowledge base for the guessed ABox is consistent and, 
therefore, a counter-model for the query entailment. 

In its (equivalent) negated form, Lemma~\ref{lem:correctness} says that 
$\KB \not\models \Q$ iff there is an extended knowledge base $\KB_\Q$ 
w.r.t.\ \KB and $\Q$ such that $\KB_\Q$ is consistent. Together with 
Lemma~\ref{lem:UNA} it follows, therefore, that the algorithm from 
Definition~\ref{def:algonondeterministic} is correct. 



\subsubsection{Data Complexity of Query Entailment in \SHIQ}
\label{sect:datacomplexity}

We now analyze the data complexity of the algorithm given in 
Definition~\ref{def:algonondeterministic} and show that deciding UCQ 
entailment in \SHIQ is indeed in co-\NPclass for data complexity. 

\begin{theorem}\label{thm:datacomplexity}
  Let \TB be a \SHIQ TBox, \RB a \SHIQ role hierarchy, and \Q a union of 
  Boolean conjunctive queries. Given a \SHIQ ABox \AB with $m_a = 
  |\AB|$, the algorithm from Definition~\ref{def:algonondeterministic} 
  decides in non-deterministic polynomial time in $m_a$ whether $\KB 
  \not\models \Q$ for \KB = (\TB, \RB, \AB). 
\end{theorem}

Clearly, the size of an ABox $\AB^\Pmc$ in an \AB-partition is bounded 
by $m_a$. Since the query is no longer an input, its size is constant 
and the transformation to CNF can be done in constant time. We then 
non-deterministically choose one of the resulting conjuncts. Let this 
conjunct be $\Q_i = \Q_{(i, 1)} \vee \ldots \vee \Q_{(i, \ell)}$. As 
established in Lemma~\ref{thm:combinedcomplexity}, the maximal size of 
an extended ABox $\AB^\Pmc_{\Q_i}$ is polynomial in $m_a$. Hence, 
$|\AB^\Pmc \cup \AB^\Pmc_{\Q_i}| \leq p(m_a)$ for some polynomial $p$. 
Due to Lemma~\ref{lem:counting} and since the size of \Q, \TB, and \RB 
is fixed by assumption, the sets $\trees[\KB^\Pmc]{\Q_{(i, j)}}$ and 
$\groundings[\KB^\Pmc]{\Q_{(i, j)}}$ for each $j$ such that $1 \leq j 
\leq \ell$ can be computed in time polynomial in $m_a$. From 
Lemma~\ref{lem:combinedcomplexity}, we know that the translation of an 
extended knowledge base into an \ALCQIb knowledge base is polynomial in 
$m_a$ and a close inspection of the algorithm by \citeA{Tobi01a} for 
deciding consistency of an \ALCQIb knowledge base shows that its runtime 
is also polynomial in $m_a$.

The bound given in Theorem~\ref{thm:datacomplexity} is tight since the 
data complexity of conjunctive query entailment is already 
co-\NPclass-hard for the \ALE fragment of \SHIQ \cite{Scha93a}.

\begin{corollary}
  Conjunctive query entailment in \SHIQ is data complete for 
  co-\NPclass.
\end{corollary}

Due to the correspondence between query containment and query answering 
\cite{CaDL98a}, the algorithm can also be used to decide containment 
of two unions of conjunctive queries over a \SHIQ knowledge base, which 
gives the following result:

\begin{corollary}
  Given a \SHIQ knowledge base \KB and two unions of conjunctive queries 
  $\Q$ and $\Q'$, the problem whether $\KB \models \Q \subseteq \Q'$ is 
  decidable.
\end{corollary}

By using the result of \citeA[Thm.~11]{Rosa06a}, we further show that 
the consistency of a \SHIQ knowledge base extended with (weakly-safe) 
Datalog rules is decidable.

\begin{corollary}
  The consistency of $\SHIQ$+$log$-KBs (both under FOL semantics and 
  under NM semantics) is decidable.
\end{corollary}

==> intro.tex <==
\section{Introduction}\label{sect:intro}

Description Logics (DLs) are a family of logic based knowledge 
representation formalisms \cite{dlhb}. Most DLs are fragments of 
First-Order Logic restricted to unary and binary predicates, which are 
called concepts and roles in DLs. The constructors for building complex 
expressions are usually chosen such that the key inference problems, 
such as concept satisfiability, are decidable and preferably of low 
computational complexity. A DL knowledge base (KB) consists of a TBox, 
which contains intensional knowledge such as concept definitions and 
general background knowledge, and an ABox, which contains extensional 
knowledge and is used to describe individuals. Using a database 
metaphor, the TBox corresponds to the schema, and the ABox corresponds 
to the data. In contrast to databases, however, DL knowledge bases adopt 
an open world semantics, i.e., they represent information about the 
domain in an incomplete way. 

Standard DL reasoning services include testing concepts for 
satisfiability and retrieving certain instances of a given concept. The 
latter retrieves, for a knowledge base consisting of an ABox \AB and a 
TBox \TB, all (ABox) individuals that are instances of the given 
(possibly complex) concept expression $C$, i.e., all those individuals 
$a$ such that \TB and \AB entail that $a$ is an instance of $C$. The 
underlying reasoning problems are well-understood, and it is known that 
the combined complexity of these reasoning problems, i.e., the 
complexity measured in the size of the TBox, the ABox, and the query, is 
\ExpTime-complete for \SHIQ \cite{Tobi01a}. The data complexity of a 
reasoning problem is measured in the size of the ABox only. Whenever the 
TBox and the query are small compared to the ABox, as is often the 
case in practice, the data complexity gives a more useful performance 
estimate. For \SHIQ, instance retrieval is known to be data complete for 
co-\NPclass \cite{HuMS05a}. 

Despite the high worst case complexity of the standard reasoning 
problems for very expressive DLs such as \SHIQ, there are highly 
optimized implementations available, e.g., FaCT++ \cite{TsHo06a}, 
KAON2\footnote{\url{http://kaon2.semanticweb.org}}, Pellet 
\cite{SPGK06a}, and 
RacerPro\footnote{\url{http://www.racer-systems.com}}. These systems are 
used in a wide range of applications, e.g., configuration 
\cite{McWr98a}, bio informatics \cite{WBHL05a}, and information 
integration \cite{CDLN98a}. Most prominently, DLs are known for their 
use as a logical underpinning of ontology languages, e.g., OIL, 
DAML+OIL, and OWL \cite{HoPH03a}, which is a W3C recommendation 
\cite{BHHH04a}. 

In data-intensive applications, querying KBs plays a central role. 
Instance retrieval is, in some aspects, a rather weak form of querying: 
although possibly complex concept expressions are used as queries, we 
can only query for tree-like relational structures, i.e., a DL concept 
cannot express arbitrary cyclic structures. This property is known as 
the tree model property and is considered an important reason for the 
decidability of most Modal and Description Logics 
\cite{Grad01a,Vard97a}. Conjunctive queries (CQs) are well known in the 
database community and constitute an expressive query language with 
capabilities that go well beyond standard instance retrieval. For an 
example, consider a knowledge base that contains an ABox assertion 
$(\exists \dlf{hasSon}.(\exists \dlf{hasDaughter}.\top))(\dlf{Mary})$, 
which informally states that the individual (or constant in FOL terms) 
Mary has a son who has a daughter; hence, that Mary is a grandmother. 
Additionally, we assume that both roles $\dlf{hasSon}$ and 
$\dlf{hasDaughter}$ have a transitive super-role $\dlf{hasDescendant}$. 
This implies that $\dlf{Mary}$ is related via the role 
$\dlf{hasDescendant}$ to her (anonymous) grandchild. For this knowledge 
base, $\dlf{Mary}$ is clearly an answer to the conjunctive query 
$\dlf{hasSon}(x, y) \wedge \dlf{hasDaughter}(y, z) \wedge 
\dlf{hasDescendant}(x, z)$, when we assume that $x$ is a distinguished 
variable (also called answer or free variable) and $y, z$ are 
non-distinguished (existentially quantified) variables. 

%Please note that the query is considered as a cyclic query 
%since, in the presence of inverse roles, we do not consider the 
%direction given by the roles. The query can, therefore, not directly be 
%expressed as a concept.  

If all variables in the query are non-distinguished, the query answer is 
just $\dlf{true}$ or $\dlf{false}$ and the query is called a Boolean 
query. Given a knowledge base \KB and a Boolean CQ \Q, the query 
entailment problem is deciding whether \Q is $\dlf{true}$ or 
$\dlf{false}$ w.r.t.\ \KB. If a CQ contains distinguished variables, the 
answers to the query are those tuples of individual names for which the 
knowledge base entails the query that is obtained by replacing the free 
variables with the individual names in the answer tuple. The problem of 
finding all answer tuples is known as query answering. Since query 
entailment is a decision problem and thus better suited for complexity 
analysis than query answering, we concentrate on query entailment. This 
is no restriction since query answering can easily be reduced to query 
entailment as we illustrate in more detail in 
Section~\ref{pre:sect:cqs}. 

Devising a decision procedure for conjunctive query entailment in 
expressive DLs such as SHIQ is a challenging problem, in particular when 
transitive roles are admitted in the query \cite{GlHS06a}. In the 
conference version of this paper, we presented the first decision 
procedure for conjunctive query entailment in \SHIQ. In this paper, we 
generalize this result to unions of conjunctive queries (UCQs) over 
\SHIQ knowledge bases. We achieve this by rewriting a conjunctive query 
into a set of conjunctive queries such that each resulting query is 
either tree-shaped (i.e., it can be expressed as a concept) or grounded 
(i.e., it contains only constants/individual names and no variables). 
The entailment of both types of queries can be reduced to standard 
reasoning problems \cite{HoTe00a,CaDL98a}. 

The paper is organized as follows: in Section~\ref{sect:preliminaries}, 
we give the necessary definitions, followed by a discussion of related 
work in Section~\ref{sect:rw}. In Section~\ref{sect:example}, we 
motivate the query rewriting steps by means of an example. In 
Section~\ref{sect:rewriting}, we give formal definitions for the 
rewriting procedure and show that a Boolean query is indeed entailed by 
a knowledge base \KB iff the disjunction of the rewritten queries is 
entailed by \KB. In Section~\ref{sect:decisionprocedure}, we present a 
deterministic algorithm for UCQ entailment in \SHIQ that runs in time 
single exponential in the size of the knowledge base and double 
exponential in the size of the query. Since the combined complexity of 
conjunctive query entailment is already 2\ExpTime-hard for the DL \ALCI 
\cite{Lutz07a}, it follows that this problem is 2\ExpTime-complete for 
\SHIQ. This shows that conjunctive query entailment for \SHIQ is 
strictly harder than instance checking, which is also the case for 
simpler DLs such as \EL \cite{Rosa07a}. We further show that (the 
decision problem corresponding to) conjunctive query answering in \SHIQ 
is co-\NPclass-complete regarding data complexity, and thus not harder 
than instance retrieval.

The presented decision procedure gives not only insight into query 
answering; it also has an immediate consequence on the field of 
extending DL knowledge bases with rules. From the work by 
\citeA[Thm.~11]{Rosa06a}, the consistency of a \SHIQ knowledge base 
extended with (weakly-safe) Datalog rules is decidable iff the 
entailment of unions of conjunctive queries in \SHIQ is decidable. 
Hence, we close this open problem as well. 

This paper is an extended version of the conference paper: Conjunctive 
Query Answering for the Description Logic \SHIQ. Proceedings of the 
Twentieth International Joint Conference on Artificial Intelligence 
(IJCAI'07), Jan 06 - 12, 2007.



==> preliminaries.tex <==
\section{Preliminaries}\label{sect:preliminaries}

We introduce the basic terms and notations used throughout the paper. In 
particular, we introduce the DL \SHIQ \cite{HoST00a} and (unions of) 
conjunctive queries. 


\subsection{Syntax and Semantics of \SHIQ}

Let \NC, \NR, and \NI be countably infinite sets of \emph{concept 
names}, \emph{role names}, and \emph{individual names}. We assume that 
the set of role names contains a subset $\NtR \subseteq \NR$ of 
\emph{transitive role names}. A \emph{role} is an element of $\NR \cup 
\{r^- \mid r \in \NR\}$, where roles of the form $r^-$ are called 
\emph{inverse roles}. A \emph{role inclusion} is of the form $r 
\sqsubseteq s$ with $r, s$ roles. A \emph{role hierarchy} \RB is a 
finite set of role inclusions.
  
An \emph{interpretation} \I = \inter consists of a non-empty set \dom, 
the \emph{domain} of \I, and a function \Int{$\cdot$}, which maps every 
concept name $A$ to a subset $\Int{A} \subseteq \dom$, every role name 
$r \in \NR$ to a binary relation $\Int{r} \subseteq \dom \times \dom$, 
every role name $r \in \NtR$ to a transitive binary relation $\Int{r} 
\subseteq \dom \times \dom$, and every individual name $a$ to an element 
$\Int{a} \in \dom$. An interpretation \I \emph{satisfies} a role 
inclusion $r \sqsubseteq s$ if $\Int{r} \subseteq \Int{s}$ and a role 
hierarchy \RB if it satisfies all role inclusions in \RB. 

We use the following standard notation:
\begin{enumerate} 
  \item 
    We define the function \mn{Inv} over roles as $\inv{r} := r^-$ if $r 
    \in \NR$ and $\inv{r} := s$ if $r = s^-$ for a role name~$s$.
  \item 
    For a role hierarchy \RB, we define \sssR as the reflexive 
    transitive closure of $\sqsubseteq$ over $\RB \cup \{\inv{r} 
    \sqsubseteq \inv{s} \mid r \sqsubseteq s \in \RB\}$. We use $r 
    \equiv_\RB s$ as an abbreviation for $r \sssR s$ and $s \sssR r$.  
  \item 
    For a role hierarchy \RB and a role $s$, we define the set $\transR$ 
    of transitive roles as $\{s \mid \mbox{there is a role } r \mbox{ 
    with } r \equiv_\RB s \mbox{ and } r \in \NtR \mbox{ or } \inv{r} 
    \in \NtR\}$. 
  \item 
    A role $r$ is called \emph{simple} w.r.t.\ a role hierarchy \RB if, 
    for each role $s$ such that \ $s \sssR r$, $s \notin \transR$. 
\end{enumerate}
The subscript \RB of \sssR and \transR is dropped if clear from the 
context. The set of $\SHIQ$\emph{-concepts} (or concepts for short) is 
the smallest set built inductively from \NC using the following grammar, 
where $A \in \NC$, $n \in \Nbbm$, $r$ is a role and $s$ is a simple 
role:
$$
  C ::= \top \mid \bot \mid A \mid \neg C \mid C_1 \sqcap C_2 \mid 
        C_1 \sqcup C_2 \mid \forall r.C \mid \exists r.C \mid 
        \leqslant n\; s.C \mid \geqslant n\; s.C.
$$

Given an interpretation \I, the semantics of $\SHIQ$-concepts is defined 
as follows:
$$
  {\setlength\arraycolsep{0.2em}
  \begin{array}{r l r l r l}
    \Int{\top} = & \dom\hspace*{.5cm}& 
    \Int{(C \sqcap D)} = & \Int{C} \cap \Int{D}\hspace*{.5cm}& 
    \Int{(\neg C)} = & \dom \setminus \Int{C}\hspace*{.5cm}\\
    \Int{\bot} = & \emptyset\hspace*{.5cm}& 
    \Int{(C \sqcup D)} = & \Int{C} \cup \Int{D}\hspace*{.5cm}& 
    \\ 
    \Int{(\forall r.C)} = & 
    \multicolumn{5}{l}{\{d \in \dom \mid \mbox{ if } (d, d') \in 
    \Int{r}, \mbox{ then } d' \in \Int{C}\}}\\
    \Int{(\exists r.C)} = & 
    \multicolumn{5}{l}{\{d \in \dom \mid \mbox{ there is a } (d, d') 
    \in \Int{r} \mbox{ with } d' \in \Int{C}\}}\\
    \Int{(\leqslant n\; s.C)} = & \multicolumn{5}{l}{\{d \in \dom 
      \mid \card{\Int{s}(d, C)} \leq n\}}\\
    \Int{(\geqslant n\; s.C)} = & \multicolumn{5}{l}{\{d \in \dom 
      \mid \card{\Int{s}(d, C)} \geq n\}}\\
  \end{array}
  }
$$
where $\card{M}$ denotes the cardinality of the set $M$ and $\Int{s}(d,
C)$ is defined as 
$$
  \{d' \in \dom \mid (d, d') \in \Int{s} \mbox{ and } d' \in \Int{C}\}.
$$

A \emph{general concept inclusion} (GCI) is an expression $C \sqsubseteq 
D$, where both $C$ and $D$ are concepts. A finite set of GCIs is called 
a \emph{TBox}. An interpretation \I \emph{satisfies} a GCI $C 
\sqsubseteq D$ if $\Int{C} \subseteq \Int{D}$, and a TBox \TB if it 
satisfies each GCI in \TB. 

An (ABox) \emph{assertion} is an expression of the form $C(a)$, $r(a, 
b)$, $\neg r(a,b)$, or $a \ndoteq b$, where $C$ is a concept, $r$ is a 
role, $a, b \in \NI$. An \emph{ABox} is a finite set of assertions. We 
use \indA to denote the set of individual names occurring in \AB. An 
interpretation \I \emph{satisfies} an assertion $C(a)$ if $\Int{a} \in 
\Int{C}$, $r(a, b)$ if $(\Int{a}, \Int{b}) \in \Int{r}$, $\neg r(a, b)$ 
if $(\Int{a}, \Int{b}) \notin \Int{r}$, and $a \ndoteq b$ if $\Int{a} 
\neq \Int{b}$. An interpretation \I \emph{satisfies} an ABox if it 
satisfies each assertion in \AB, which we denote with $\I \models \AB$.

A \emph{knowledge base} (KB) is a triple (\TB, \RB, \AB{}) with \TB a 
TBox, \RB a role hierarchy, and \AB an ABox. Let \KBDef be a KB and \I = 
\inter an interpretation. We say that \emph{\I satisfies $\KB$} if \I 
satisfies \TB, \RB, and \AB. In this case, we say that \I is a 
\emph{model} of \KB and write $\I \models \KB$.  We say that \emph{\KB 
is consistent} if \KB has a model.




\subsubsection{Extending \SHIQ to \SHIQR}

In the following section, we show how we can reduce a conjunctive query 
to a set of ground or tree-shaped conjunctive queries. During the 
reduction, we may introduce concepts that contain an intersection of 
roles under existential quantification. We define, therefore, the 
extension of \SHIQ with role conjunction/intersection, denoted as \SHIQR 
and, in the appendix, we show how to decide the consistency of \SHIQR 
knowledge bases. 

In addition to the constructors introduced for \SHIQ, \SHIQR allows for 
concepts of the form 
$$
  C ::= \forall R.C \mid \exists R.C \mid \leqslant n\; S.C \mid 
        \geqslant n\; S.C,
$$
where $R := r_1 \sqcap \ldots \sqcap r_n$, $S := s_1 \sqcap \ldots 
\sqcap s_n$, $r_1, \ldots, r_n$ are roles, and $s_1, \ldots, s_n$ are 
simple roles. The interpretation function is extended such that 
$\Int{(r_1 \sqcap \ldots \sqcap r_n)} = \Int{r_1} \cap \ldots \cap 
\Int{r_n}$. 



\subsection{Conjunctive Queries and Unions of Conjunctive Queries}
\label{pre:sect:cqs}

We now introduce Boolean conjunctive queries since they are the basic 
form of queries we are concerned with. We later also define non-Boolean 
queries and show how they can be reduced to Boolean queries. Finally, 
unions of conjunctive queries are just a disjunction of conjunctive 
queries. 

For simplicity, we write a conjunctive query as a set instead of as a 
conjunction of atoms. For example, we write the introductory example 
from Section~\ref{sect:intro} as 
$$
\{\dlf{hasSon}(x, y), \dlf{hasDaughter}(y, z), \dlf{hasDescendant}(x, 
z)\}.
$$ 

For non-Boolean queries, i.e., when we consider the problem of query 
answering, the answer variables are often given in the head of the 
query, e.g., 
$$
(x_1, x_2, x_3) \leftarrow \{\dlf{hasSon}(x_1, x_2), 
\dlf{hasDaughter}(x_2, x_3), 
\dlf{hasDescendant}(x_1, x_3)\}
$$ 
indicates that the query answers are those tuples $(a_1, a_2, a_3)$ of 
individual names that, substituted for $x_1, x_2$, and $x_3$ 
respectively, result in a Boolean query that is entailed by the 
knowledge base. For simplicity and since we mainly focus on query 
entailment, we do not use a query head even in the case of a non-Boolean 
query. Instead, we explicitly say which variables are answer variables 
and which ones are existentially quantified. We now give a definition of 
Boolean conjunctive queries. 
 
\begin{definition}
  Let \NV be a countably infinite set of variables disjoint from \NC, 
  \NR, and \NI. A \emph{term} $t$ is an element from $\NV \cup \NI$. Let 
  $C$ be a concept, $r$ a role, and $t, t'$ terms. An \emph{atom} is an 
  expression $C(t)$, $r(t, t')$, or $t \approx t'$ and we refer to these 
  three different types of atoms as \emph{concept atoms, role atoms}, 
  and \emph{equality atoms} respectively. A \emph{Boolean conjunctive 
  query} \Q is a non-empty set of atoms. We use \vars{\Q} to denote 
  the set of (existentially quantified) variables occurring in \Q, 
  \inds{\Q} to denote the set of individual names occurring in \Q, and 
  \terms{\Q} for the set of terms in \Q, where $\terms{\Q} = \vars{\Q} 
  \cup \inds{\Q}$. If all terms in \Q are individual names, we say 
  that \Q is \emph{ground}. A \emph{sub-query} of \Q is simply a 
  subset of \Q (including \Q itself). As usual, we use $\card{\Q}$ to 
  denote the cardinality of \Q, which is simply the number of atoms in 
  \Q, and we use $|\Q|$ for the size of \Q, i.e., the number of 
  symbols necessary to write \Q. A \SHIQ conjunctive query is a 
  conjunctive query in which all concepts $C$ that occur in a concept 
  atom $C(t)$ are $\SHIQ$-concepts. 

  Since equality is reflexive, symmetric and transitive, we define 
  \sapprox as the transitive, reflexive, and symmetric closure of 
  $\approx$ over the terms in \Q. Hence, the relation \sapprox is an 
  equivalence relation over the terms in \Q and, for $t \in \terms{\Q}$, 
  we use $[t]$ to denote the equivalence class of $t$ by \sapprox. 
  
  Let \I = \inter be an interpretation. A total function $\pi \colon 
  \terms{\Q} \to  \dom$ is an \emph{evaluation} if (i) $\pi(a) = 
  \Int{a}$ for each individual name $a \in \inds{\Q}$ and (ii) $\pi(t) = 
  \pi(t')$ for all $t \sapprox t'$. We write 
  \begin{itemize}
    \item 
      $\I \models^\pi C(t)$ if $\pi(t) \in \Int{C}$;
    \item 
      $\I \models^\pi r(t, t')$ if $(\pi(t), \pi(t')) \in \Int{r}$;
    \item 
      $\I \models^\pi t \approx t'$ if $\pi(t) = \pi(t')$.
  \end{itemize}
  If, for an evaluation $\pi$, $\I \models^\pi at$ for all atoms $at \in 
  \Q$, we write $\I \models^\pi \Q$. We say that \I \emph{satisfies} \Q 
  and write $\I \models \Q$ if there exists an evaluation $\pi$ such 
  that $\I \models^\pi \Q$. We call such a $\pi$ a \emph{match} for \Q 
  in \I.
  
  Let \KB be a \SHIQ knowledge base and \Q a conjunctive query. If $\I 
  \models \KB$ implies $\I \models \Q$, we say that \KB \emph{entails} 
  \Q and write $\KB \models \Q$. 
\end{definition}

The \emph{query entailment problem} is defined as follows: given a 
knowledge base \KB and a query \Q, decide whether $\KB \models \Q$. 

For brevity and simplicity of notation, we define the relation \din over 
atoms in \Q as follows: $C(t) \din \Q$ if there is a term $t' \in 
\terms{\Q}$ such that $t \sapprox t'$ and $C(t') \in \Q$, and $r(t_1, 
t_2) \din \Q$ if there are terms $t_1', t_2' \in \terms{\Q}$ such that 
$t_1 \sapprox t_1'$, $t_2 \sapprox t_2'$, and $r(t_1', t_2') \in \Q$ or 
$\inv{r}(t_2', t_1') \in \Q$. This is clearly justified by definition of 
the semantics, in particular, because $\I \models r(t, t')$ implies that 
$\I \models \inv{r}(t', t)$.

When devising a decision procedure for CQ entailment, most complications 
arise from cyclic queries \cite{CaDL98a,CaRa97a}. In this context, when 
we say cyclic, we mean that the graph structure induced by the query is 
cyclic, i.e., the graph obtained from \Q such that each term is 
considered as a node and each role atom induces an edge. Since, in the 
presence of inverse roles, a query containing the role atom $r(t, t')$ 
is equivalent to the query obtained by replacing this atom with 
$\inv{r}(t', t)$, the direction of the edges is not important and we say 
that a query is cyclic if its underlying undirected graph structure is 
cyclic. Please note also that multiple role atoms for two terms are not 
considered as a cycle, e.g., the query $\{r(t, t'), s(t, t')\}$ is not a 
cyclic query. The following is a more formal definition of this 
property. 

\begin{definition}\label{def:cyclic}
  A query \Q is \emph{cyclic} if there exists a sequence of terms $t_1, 
  \dots, t_n$ with $n > 3$ such that 
  \begin{enumerate}
    \item 
      for each $i$ with $1 \leq i < n$, there exists a role atom 
      $r_i(t_i, t_{i+1}) \din \Q$,
    \item
       $t_1 = t_n$, and 
    \item\label{it:multiedge} 
      $t_i \neq t_j$ for $1 \leq i < j < n$.
  \end{enumerate}
  \mathdefend
\end{definition}

In the above definition, Item~\ref{it:multiedge} makes sure that we do 
not consider queries as cyclic just because they contain two terms $t, 
t'$ for which there are more than two role atoms using the two terms. 
Please note that we use the relation \din here, which implicitly uses 
the relation \sapprox and abstracts from the directedness of role atoms. 
 
In the following, if we write that we replace $r(t, t') \din \Q$ with 
$s(t_1, t_2), \ldots, s(t_{n-1}, t_n)$ for $t = t_1$ and $t' = t_n$, we 
mean that we first remove any occurrences of $r(\hat{t}, \hat{t'})$ and 
$\inv{r}(\hat{t'}, \hat{t}) $ such that $\hat{t} \sapprox t$ and 
$\hat{t'} \sapprox t'$ from \Q, and then add the atoms $s(t_1, t_2), 
\ldots, s(t_{n-1}, t_n)$ to \Q. 

W.l.o.g., we assume that queries are connected. More precisely, let \Q 
be a conjunctive query. We say that \Q is \emph{connected} if, for all 
$t, t' \in \terms{\Q}$, there exists a sequence $t_1, \dots, t_n$ such 
that $t_1 = t$, $t_n = t'$ and, for all $1 \leq i < n$, there exists a 
role $r$ such that $r(t_i, t_{i+1}) \din \Q$. A collection $\Q_1, 
\dots, \Q_n$ of queries is a \emph{partitioning} of \Q if $\Q = \Q_1 
\cup \ldots \cup \Q_n$, $\Q_i \cap \Q_j = \emptyset$ for $1 \leq i 
< j \leq n$, and each $\Q_i$ is connected. 

\begin{lemma}
  Let \KB be a knowledge base, \Q a conjunctive query, and $\Q_1, \dots, 
  \Q_n$ a partitioning of $\Q$. Then $\KB \models \Q$ iff $\KB \models 
  \Q_i$ for each $i$ with $1 \leq i \leq n$.
\end{lemma}

A proof is given by \citeA[7.3.2]{Tess01a} and, with this lemma, it is 
clear that the restriction to connected queries is indeed w.l.o.g.\ 
since entailment of \Q can be decided by checking entailment of each 
$\Q_i$ at a time. In what follows, we therefore assume queries to be 
connected without further notice.

\begin{definition}
  A \emph{union of Boolean conjunctive queries} is a formula $\Q_1 \vee 
  \ldots \vee \Q_n$, where each disjunct $\Q_i$ is a Boolean conjunctive 
  query. 
  
  A knowledge base \KB \emph{entails} a union of Boolean conjunctive 
  queries $\Q_1 \vee \ldots \vee \Q_n$, written as $\KB \models \Q_1 
  \vee \ldots \vee \Q_n$, if, for each interpretation \I such that $\I 
  \models \KB$, there is some $i$ such that $\I \models \Q_i$ and $1 
  \leq i \leq n$. 
\end{definition}

W.l.o.g.\ we assume that the variable names in each disjunct are 
different from the variable names in the other disjuncts. This can 
always be achieved by naming variables apart. We further assume that 
each disjunct is a connected conjunctive query. This is w.l.o.g. since a 
UCQ which contains unconnected disjuncts can always be transformed into 
conjunctive normal form; we can then decide entailment for each 
resulting conjunct separately and each conjunct is a union of connected 
conjunctive queries. We describe this transformation now in more detail 
and, for a more convenient notation, we write a conjunctive query 
$\{at_1, \ldots, at_k\}$ as $at_1 \wedge \ldots \wedge at_k$ in the 
following proof, instead of the usual set notation. 

\begin{lemma}\label{lem:cnf}
  Let \KB be a knowledge base, $\Q = \Q_1 \vee \ldots \vee \Q_n$ a union 
  of conjunctive queries such that, for $1 \leq i \leq n, \Q_i^1, 
  \ldots, \Q_i^{k_i}$ is a partitioning of the conjunctive query $\Q_i$. 
  Then $\KB \models \Q$ iff 
  $$
  \KB \models \bigwedge\limits_{(i_1, \ldots, i_n) \in \{1, \ldots, 
  k_1\} \times \ldots \times \{1, \ldots, k_n\}} (\Q_1^{i_1} \vee \ldots 
  \vee \Q_n^{i_n}). 
  $$
  % (\Q_1^1 \vee \ldots \vee \Q_n^1) \wedge \ldots 
  % \wedge (\Q_1^{k_1} \vee \ldots \vee \Q_n^{k_n})$.
\end{lemma}

Again, a detailed proof is given by \citeA[7.3.3]{Tess01a}. Please note 
that, due to the transformation into conjunctive normal form, the 
resulting number of unions of connected conjunctive queries for which we 
have to test entailment can be exponential in the size of the original 
query. When analysing the complexity of the decision procedures 
presented in Section~\ref{sect:decisionprocedure}, we show that the 
assumption that each CQ in a UCQ is connected does not increase the 
complexity. 

We now make the connection between query entailment and query answering 
clearer. For query answering, let the variables of a conjunctive query 
be typed: each variable can either be existentially quantified (also 
called \emph{non-distinguished}) or free (also called 
\emph{distinguished} or \emph{answer variables}). Let \Q be a query in 
$n$ variables (i.e., $\card{\vars{\Q}} = n$), of which $v_1, \dots, v_m$ 
($m \leq n$) are answer variables. The \emph{answers} of \KBDef to 
\Q are those $m$-tuples $(a_1, \dots, a_m) \in \indA^m$ such that, for 
all models \I of \KB, $\I \models^\pi \Q$ for some $\pi$ that satisfies 
$\pi(v_i) = \Int{a_i}$ for all $i$ with $1 \leq i \leq m$. It 
is not hard to see that the answers of \KB to \Q can be computed by 
testing, for each $(a_1, \ldots, a_m) \in \indA^m$, whether the query 
$\Q_{[v_1, \dots, v_m/a_1, \ldots, a_m]}$ obtained from \Q by replacing 
each occurrence of $v_i$ with $a_i$ for $1 \leq i \leq m$ is 
entailed by \KB. The answer to \Q is then the set of all $m$-tuples 
$(a_1, \ldots, a_m)$ for which $\KB \models \Q_{[v_1, \dots, v_m/a_1, 
\ldots, a_m]}$. Let $k = \card{\indA}$ be the number of individual names 
used in the ABox \AB. Since \AB is finite, clearly $k$ is finite. Hence, 
deciding which tuples belong to the set of answers can be checked with 
at most $k^m$ entailment tests. This is clearly not very efficient, but 
optimizations can be used, e.g., to identify a (hopefully small) set of 
candidate tuples. 

The algorithm that we present in Section~\ref{sect:decisionprocedure} 
decides query entailment. The reasons for devising a decision procedure 
for query entailment instead of query answering are two-fold: first, 
query answering can be reduced to query entailment as shown above; 
second, in contrast to query answering, query entailment is a decision 
problem and can be studied in terms of complexity theory. 

In the remainder of this paper, if not stated otherwise, we use \Q 
(possibly with subscripts) for a connected Boolean conjunctive query, 
\KB for a \SHIQ knowledge base (\TB, \RB, \AB{}), \I for an 
interpretation \inter, and $\pi$ for an evaluation. 


==> relatedWork.tex <==
\section{Related Work}
\label{sect:rw}

Very recently, an automata-based decision procedure for positive 
existential path queries over \ALCQIbreg knowledge bases has been 
presented \cite{CaEO07a}. Positive existential path queries generalize 
unions of conjunctive queries and since a \SHIQ knowledge base can be 
polynomially reduced to an \ALCQIbreg knowledge base, the presented 
algorithm is a decision procedure for (union of) conjunctive query 
entailment in \SHIQ as well. The automata-based technique can be 
considered more elegant than our rewriting algorithm, but it does not 
give an \NPclass upper bound for the data complexity as our technique. 

%gives less insight into why and how queries can always be mapped 
%to a tree- or forest-shaped model. Furthermore, our algorithm does not 
%rely on a particular reasoning method. Hence, any of the existing, 
%highly optimzed reasoner implementations can easily be extended to 
%support conjunctive queries with the technique we introduce here.

Most existing algorithms for conjunctive query answering in expressive 
DLs assume, however, that role atoms in conjunctive queries use only 
roles that are not transitive. As a consequence, the example query from 
the introductory section cannot be answered. Under this restriction, 
decision procedures for various DLs around \SHIQ are known 
\cite{HoTe00a,OrCE06a}, and it is known that answering conjunctive 
queries in this setting is data complete for 
\hbox{co-\NPclass~\cite{OrCE06a}.} Another common restriction is that 
only individuals named in the ABox are considered for the assignments of 
variables. In this setting, the semantics of queries is no longer the 
standard First-Order one. With this restriction, the answer to the 
example query from the introduction would be $\dlf{false}$ since 
$\dlf{Mary}$ is the only named individual. It is not hard to see that 
conjunctive query answering with this restriction can be reduced to 
standard instance retrieval by replacing the variables with individual 
names from the ABox and then testing the entailment of each conjunct 
separately. Most of the implemented DL reasoners, e.g., KAON2, Pellet, 
and RacerPro, provide an interface for conjunctive query answering in 
this setting and employ several optimizations to improve the performance 
\cite{SiPa06a,MoSS04a,WeMo05a}. Pellet appears to be the only reasoner 
that also supports the standard First-Order semantics for \SHIQ 
conjunctive queries under the restriction that the queries are acyclic. 

To the best of our knowledge, it is still an open problem whether 
conjunctive query entailment is decidable in \SHOIQ. Regarding 
undecidability results, it is known that conjunctive query entailment 
in the two variable fragment of First-Order Logic $\Lmc_2$ is 
undecidable \cite{Rosa07b} and Rosati identifies a relatively small 
set of constructors that causes the undecidability. 

Query entailment and answering have also been studied in the context of 
databases with incomplete information \cite{Rosa06b,Meyd98a,Grah91a}. In 
this setting, DLs can be used as schema languages, but the expressivity 
of the considered DLs is much lower than the expressivity of \SHIQ. For 
example, the constructors provided by logics of the DL-Lite family 
\cite{CDLL07a} are chosen such that the standard reasoning tasks are in 
\PTime and query entailment is in \LogSpace with respect to data 
complexity. Furthermore, TBox reasoning can be done independently of the 
ABox and the ABox can be stored and accessed using a standard database 
SQL engine. Since the considered DLs are considerable less expressive 
than \SHIQ, the techniques used in databases with incomplete information 
cannot be applied in our setting. 


%The data complexity of conjunctive query entailment in many DLs, 
%including the one we study here, is co-\NPclass-complete. For a few less 
%expressive logics such as \EL and \DLLite, however, the data complexity 
%is known to be \PTime-complete \cite{Rosa07b}. 

Regarding the query language, it is well known that an extension of 
conjunctive queries with inequalities is undecidable \cite{CaDL98a}. 
Recently, it has further been shown that even for DLs with 
low expressivity, an extension of conjunctive queries with inequalities 
or safe role negation leads to undecidability \cite{Rosa07b}. 

A related reasoning problem is \emph{query containment}. Given a schema 
(or TBox) \Smc and two queries $q$ and $q'$, we have that $q$ is 
contained in $q'$ w.r.t.\ \Smc iff every interpretation \I that 
satisfies \Smc and $q$ also satisfies $q'$. It is well known that query 
containment w.r.t.\ a TBox can be reduced to deciding query entailment 
for (unions of) conjunctive queries w.r.t.\ a knowledge base 
\cite{CaDL98a}. Hence a decision procedure for (unions of) conjunctive 
queries in \SHIQ can also be used for deciding query containment w.r.t.\ 
to a \SHIQ TBox.

Entailment of unions of conjunctive queries is also closely related to 
the problem of adding rules to a DL knowledge base, e.g., in the form of 
Datalog rules. Augmenting a DL KB with an arbitrary Datalog program 
easily leads to undecidability \cite{LeRo98a}. In order to ensure 
decidability, the interaction between the Datalog rules and the DL 
knowledge base is usually restricted by imposing a safeness condition. 
The \DLlog framework \cite{Rosa06a} provides the least restrictive 
integration proposed so far. Rosati presents an algorithm that decides 
the consistency of a \DLlog knowledge base by reducing the problem to 
entailment of unions of conjunctive queries, and he proves that 
decidability of UCQs in \SHIQ implies the decidability of consistency 
for $\SHIQ$+$log$ knowledge bases.

%\begin{theorem}{\cite[Thm. 11]{Rosa06a}} 
%  For every description logic $\mathcal{DL}$, satisfiability of 
%  \DLlog-KBs (both under FOL semantics and under NM 
%  semantics) is decidable iff Boolean UCQ containment is decidable in 
%  $\mathcal{DL}$.
%\end{theorem}


==> rewriting.tex <==
\section{Query Rewriting}\label{sect:rewriting}

In the previous section, we have used several terms, e.g., tree- or 
forest-shaped query, rather informally. In the following, we give 
definitions for the terms used in the query rewriting process. Once this 
is done, we formalize the query rewriting steps and prove the 
correctness of the procedure, i.e., we show that the forest-shaped 
queries obtained in the rewriting process can indeed be used for 
deciding whether a knowledge base entails the original query. We do not 
give the detailed proofs here, but rather some intuitions behind the 
proofs. Proofs in full detail are given in the appendix.  

\subsection{Tree- and Forest-Shaped Queries}\label{sect:queryshapes}

In order to define tree- or forest-shaped queries more precisely, we use 
mappings between queries and trees or forests. Instead of mapping 
equivalence classes of terms by \sapprox to nodes in a tree, we extend 
some well-known properties of functions as follows:

\begin{definition} 
  For a mapping $f \colon A \to B$, we use $\domain{f}$ and $\range{f}$ 
  to denote $f$'s \emph{domain} $A$ and \emph{range} $B$, respectively. 
  Given an equivalence relation \sapprox on $\domain{f}$, we say that 
  $f$ is \emph{injective modulo \sapprox} if, for all $a, a' \in 
  \domain{f}$, $f(a) = f(a')$ implies $a \sapprox a'$ and we say that 
  $f$ is \emph{bijective modulo $\sapprox$} if $f$ is injective modulo 
  \sapprox and surjective. 
%\end{definition}
%
%Let $\Q'$ be a query obtained from \Q by selecting one representative 
%term $t$ for each equivalence class such that, if $a \in [t]$ for $a \in 
%\indA$, then $a = t$ and replacing each term $t' \in [t]$ with $t$. Such 
%an $a$ is unique since for now we make the unique name assumption. By 
%definition of the semantics of conjunctive queries we have that \Q is 
%entailed by a knowledge base \KB iff $\Q'$ is entailed by \KB. It is not 
%hard to see that a mapping for \Q that is injective modulo \sapprox is 
%injective for $\Q'$. 
%
%\begin{definition}
  Let \Q be a query. A \emph{tree mapping} for \Q is a total function 
  $f$ from terms in \Q to a tree such that 
  \begin{enumerate}
    \item
      $f$ is bijective modulo \sapprox, 
    \item
      if $r(t, t') \din \Q$, then $f(t)$ is a neighbor of $f(t')$, 
      and, 
    \item
      if $a \in \inds{\Q}$, then $f(a) = \varepsilon$. 
  \end{enumerate}
  The query \Q is \emph{tree-shaped} if $\card{\inds{\Q}} \leq 1$ 
  and there is a tree mapping for \Q. 
  
  A \emph{root choice} \roots for \Q is a subset of \terms{\Q} such that 
  $\inds{\Q} \subseteq \roots$ and, if $t \in \roots$ and $t \sapprox 
  t'$, then $t' \in \roots$. For $t \in \roots$, we use $\reach{t}$ to 
  denote the set of terms $t' \in \terms{\Q}$ for which there exists a 
  sequence of terms $t_1, \dots, t_n \in \terms{\Q}$ such that 
  \begin{enumerate} 
    \item 
      $t_1 = t$ and $t_n = t'$, 
    \item 
      for all $1 \leq i < n$, there is a role $r$ such that $r(t_i, 
      t_{i+1}) \din \Q$, and,   
    \item\label{it:split} 
      for $1 < i \leq n$, if $t_i \in \roots$, then $t_i \sapprox t$.
  \end{enumerate}
  We call \roots a \emph{root splitting w.r.t.\ $\Q$} if either $\roots 
  = \emptyset$ or if, for $t_i, t_j \in \roots$, $t_i \nsapprox t_j$ 
  implies that $\reach{t_i} \cap \reach{t_j} = \emptyset$. Each term $t 
  \in \roots$ induces a sub-query 
  $$
    \begin{array}{l l} 
      \sq{\Q, t} := & \{at \din \Q \mid \mbox{ the terms in $at$ occur 
      in } \reach{t}\} \setminus \\ & 
      \{r(t, t) \mid r(t, t) \din \Q\}. 
    \end{array}
  $$ 
  A query \Q is \emph{forest-shaped w.r.t.\ a root splitting} \roots if 
  either $\roots = \emptyset$ and \Q is tree-shaped or each sub-query 
  $\sq{\Q, t}$ for $t \in \roots$ is tree-shaped. 
\end{definition}

For each term $t \in \roots$, we collect the terms that are reachable 
from $t$ in the set $\reach{t}$. By Condition~\ref{it:split}, we make 
sure that \roots and \sapprox are such that each $t' \in \reach{t}$ is 
either not in \roots or $t \sapprox t'$. Since queries are connected by 
assumption, we would otherwise collect all terms in $\reach{t}$ and not 
just those $t' \notin \roots$. For a root splitting, we require that the 
resulting sets are mutually disjoint for all terms $t, t' \in \roots$ 
that are not equivalent. This guarantees that all paths between the 
sub-queries go via the root nodes of their respective trees. 
Intuitively, a forest-shaped query is one that can potentially be mapped 
onto a canonical interpretation \I = \inter such that the terms in the 
root splitting \roots correspond to roots $(a, \varepsilon) \in \dom$. 
In the definition of $\sq{\Q, t}$, we exclude loops of the form $r(t, t) 
\din \Q$, as these parts of the query are grounded later in the query 
rewriting process and between ground terms, we allow arbitrary 
relationships. 

Consider, for example, the query $\Q_{sr}$ of our running example from 
the previous section (cf.\ Figure~\ref{fig:splitrewriting}). Let us 
again make the root choice $\roots := \{ux, x\}$ for \Q. The sets 
$\reach{ux}$ and $\reach{x}$ w.r.t.\ $\Q_{sr}$ and \roots are $\{ux, 
u\}$ and $\{x, y, z\}$ respectively. Since both sets are disjoint, 
\roots is a root splitting w.r.t.\ $\Q_{sr}$. If we choose, however, 
$\roots := \{x, y\}$, the set \roots is not a root splitting w.r.t.\ 
$\Q_{sr}$ since $\reach{x} = \{ux, u, z\}$ and $\reach{y} = \{z\}$ are 
not disjoint.



\subsection{From Graphs to Forests}\label{sect:rewritingsteps}

We are now ready to define the query rewriting steps. Given an arbitrary 
query, we exhaustively apply the rewriting steps and show that we can 
use the resulting queries that are forest-shaped for deciding entailment 
of the original query. Please note that the following definitions are 
for conjunctive queries and not for unions of conjunctive queries since 
we apply the rewriting steps for each disjunct separately. 

\begin{definition}\label{def:rewriting}
  Let \Q be a Boolean conjunctive query. A \emph{collapsing} $\Q_{co}$ 
  of \Q is obtained by adding zero or more equality atoms of the form 
  $t \approx t'$ for $t, t' \in \terms{\Q}$ to \Q. We use \co{\Q} to 
  denote the set of all queries that are a collapsing of \Q. 
  
  Let \KB be a \SHIQ knowledge base. A query $\Q_{sr}$ is called a 
  \emph{split rewriting} of \Q w.r.t.\ \KB if it is obtained from \Q by 
  choosing, for each atom $r(t, t') \din \Q$, to either:
  \begin{enumerate}
    \item 
      do nothing,
    \item 
      choose a role $s \in \transR$ such that $s \sssR r$ and replace 
      $r(t, t')$ with $s(t, u), s(u, t')$, or 
    \item 
      choose a role $s \in \transR$ such that $s \sssR r$ and replace 
      $r(t, t')$ with $s(t, u)$, $s(u, u')$, $s(u', t')$, 
  \end{enumerate}
  where $u, u' \in \NV$ are possibly fresh variables. We use \srK{\Q} to 
  denote the set of all pairs $(\Q_{sr}, \roots)$ for which there is a 
  query $\Q_{co} \in \co{\Q}$ such that $\Q_{sr}$ is a split rewriting 
  of $\Q_{co}$ and \roots is a root splitting w.r.t.\ $\Q_{sr}$.
  
  A query $\Q_{\ell r}$ is called a \emph{loop rewriting} of \Q w.r.t.\ 
  a root splitting \roots and \KB if it is obtained from \Q by choosing, 
  for all atoms of the form $r(t, t) \din \Q$ with $t \notin \roots$, a 
  role $s \in \transR$ such that $s \sssR r$ and by replacing $r(t, t)$ 
  with two atoms $s(t, t')$ and $s(t', t)$ for $t' \in \NV$ a possibly 
  fresh variable. We use \lrK{\Q} to denote the set of all pairs 
  $(\Q_{\ell r}, \roots)$ for which there is a tuple $(\Q_{sr}, \roots) 
  \in \srK{\Q}$ such that $\Q_{\ell r}$ is a loop rewriting of $\Q_{sr}$ 
  w.r.t.\ \roots and \KB.

  For a forest rewriting, fix a set $V \subseteq \NV$ of variables not 
  occurring in \Q such that $\card{V} \leq \card{\vars{\Q}}$. A 
  \emph{forest rewriting} $\Q_{fr}$ w.r.t.\ a root splitting \roots of 
  \Q and \KB is obtained from \Q by choosing, for each role atom $r(t, 
  t')$ such that either $\roots = \emptyset$ and $r(t, t') \din \Q$ or 
  there is some $t_r \in \roots$ and $r(t, t') \din \sq{\Q, t_r}$ to 
  either 
  \begin{enumerate}
    \item 
      do nothing, or
    \item
      choose a role $s \in \transR$ such that $s \sssR r$ and replace 
      $r(t, t')$ with $\ell \leq \card{\vars{\Q}}$ role atoms $s(t_1, 
      t_2), \ldots, s(t_\ell, t_{\ell + 1})$, where $t_1 = t$, $t_{\ell 
      + 1} = t'$, and $t_2, \ldots, t_\ell \in \vars{\Q} \cup V$.
  \end{enumerate}
  We use \frK{\Q} to denote the set of all pairs $(\Q_{fr}, \roots)$ for 
  which there is a tuple $(\Q_{\ell r}, \roots) \in \lrK{\Q}$ such that 
  $\Q_{fr}$ is a forest-shaped forest rewriting of $\Q_{\ell r}$ w.r.t.\ 
  \roots and \KB. 
\end{definition}

If \KB is clear from the context, we say that $\Q'$ is a split, loop, or 
forest rewriting of \Q instead of saying that $\Q'$ is a split, loop, or 
forest rewriting of \Q w.r.t.\ \KB. We assume that $\srK{\Q}, \lrK{\Q}$, 
and $\frK{\Q}$ contain no isomorphic queries, i.e., differences in 
(newly introduced) variable names only are neglected.

In the next section, we show how we can build a disjunction of 
conjunctive queries $\Q_1 \vee \cdots \vee \Q_\ell$ from the queries in 
\frK{\Q} such that each $\Q_i$ for $1 \leq i \leq \ell$ is 
either of the form $C(v)$ for a single variable $v \in \vars{\Q_i}$ or 
$\Q_i$ is ground, i.e., $\Q_i$ contains only constants and no variables. 
It then remains to show that $\KB \models \Q$ iff $\KB \models \Q_1 \vee 
\cdots \vee \Q_\ell$.



\subsection{From Trees to Concepts}
\label{sect:rollingup}

In order to transform a tree-shaped query into a single concept atom and 
a forest-shaped query into a ground query, we define a mapping $f$ from 
the terms in each tree-shaped sub-query to a tree. We then incrementally 
build a concept that corresponds to the tree-shaped query by traversing 
the tree in a bottom-up fashion, i.e., from the leaves upwards to the 
root. 

\begin{definition}\label{def:rollingUp}
  Let \Q be a tree-shaped query with at most one individual name. If $a 
  \in \inds{\Q}$, then let $t_r = a$ otherwise let $t_r = v$ for some 
  variable $v \in \vars{\Q}$. Let $f$ be a tree mapping such that 
  $f(t_r) = \varepsilon$. We now inductively assign, to each term $t \in 
  \terms{\Q}$, a concept $\con{\Q, t}$ as follows:
  \begin{itemize}
    \item 
      if $f(t)$ is a leaf of $\range{f}$, then $\con{\Q, t} := 
      \bigsqcap_{C(t) \din \Q} C$,
    \item 
      if $f(t)$ has successors $f(t_1), \dots, f(t_k)$, then  
      $$
      \begin{array}{l l}
        \con{\Q, t} := 
        & \bigsqcap_{C(t) \din \Q} C \, \sqcap \\[.5em]
        & \bigsqcap_{1 \leq i \leq k} \exists \big( 
          \bigsqcap_{r(t, t_i) \din \Q} r \big) . \con{\Q, t_i}.\\
      \end{array}
      $$
  \end{itemize}
  Finally, the \emph{query concept of \Q w.r.t.\ $t_r$} is 
  $\con{\Q, t_r}$.
\end{definition}

Please note that the above definition takes equality atoms into account. 
This is because the function $f$ is bijective modulo $\sapprox$ and, in 
case there are concept atoms $C(t)$ and $C(t')$ for $t \sapprox t'$, 
both concepts are conjoined in the query concept due to the use of the 
relation $\din$. Similar arguments can be applied to the role atoms. 

The following lemma shows that query concepts indeed capture the 
semantics of \Q.

\begin{lemma}\label{lem:conceptsandqueries}
  Let \Q be a tree-shaped query with $t_r \in \terms{\Q}$ as defined 
  above, $C_\Q = \con{\Q, t_r}$, and \I an interpretation. Then $\I 
  \models \Q$ iff there is a match $\pi$ and an element $d \in 
  \Int{C_\Q}$ such that $\pi(t_r) = d$.
\end{lemma} 

The proof given by \citeA{HSTT99a} easily transfers from \DLR to \SHIQ. 
By applying the result from the above lemma, we can now transform a 
forest-shaped query into a ground query as follows:

\begin{definition}\label{def:transformations}
  Let $(\Q_{fr}, \roots) \in \frK{\Q}$ for $\roots \neq \emptyset$, and 
  $\tau \colon \roots \to \indA$ a total function such that, for each $a 
  \in \inds{\Q}$, $\tau(a) = a$ and, for $t, t' \in \roots$, $\tau(t) = 
  \tau(t')$ iff $t \sapprox t'$. We call such a mapping $\tau$ a 
  \emph{ground mapping for \roots w.r.t.\ $\AB$}. We obtain a ground 
  query $\grounding{\Q_{fr}, \roots, \tau}$ of $\Q_{fr}$ w.r.t.\ the 
  root splitting \roots and ground mapping $\tau$ as follows:
  \begin{itemize}
    \item 
      replace each $t \in \roots$ with $\tau(t)$, and, 
    \item
      for each $a \in \range{\tau}$, replace the sub-query $\Q_a = 
      \sq{\Q_{fr}, a}$ with $\con{\Q_a, a}$.
  \end{itemize}
  We define the set \groundings{\Q} of \emph{ground queries for} \Q 
  w.r.t.\ \KB as follows: 
  $$
  \begin{array}{l l}
    \groundings{\Q} := \{\Q' \mid 
    & \mbox{there exists some }(\Q_{fr}, \roots) \in \frK{\Q} 
            \mbox{ with } \roots \neq \emptyset \\
    & \mbox{and some ground mapping $\tau$ w.r.t.\ \AB and \roots} \\
    & \mbox{such that } \Q' = \grounding{\Q_{fr}, \roots, \tau}\}
  \end{array}
  $$
  We define the set of \trees{\Q} of \emph{tree queries for} \Q as 
  follows:
  $$
  \begin{array}{l l}
    \trees{\Q} := \{\Q' \mid 
    & \mbox{there exists some }(\Q_{fr}, \emptyset) \in \frK{\Q} 
      \mbox{ and }\\
    &  v \in \vars{\Q_{fr}} \mbox{ such that } \Q' = (\con{\Q_{fr}, 
       v})(v)\}\\
  \end{array}
  $$
  \mathdefend
\end{definition}

Going back to our running example, we have already seen that $(\Q_{fr}, 
\{ux, x\})$ belongs to the set \frK{\Q} for 
$$ 
\Q_{fr} = \{r(u, ux), r(ux, x), r(x, y), t(y, y'), t(y', y), s(z, y), 
r(y, z)\}. 
$$ 
There are also several other queries in the set \frK{\Q}, e.g., $(\Q, 
\{u, x, y, z\})$, where \Q is the original query and the root splitting 
\roots is such that $\roots = \terms{\Q}$, i.e., all terms are in the 
root choice for \Q. In order to build the set $\groundings{\Q}$, we now 
build all possible ground mappings $\tau$ for the set \indA of 
individual names in our ABox and the root splittings for the queries in 
\frK{\Q}. The tuple $(\Q_{fr}, \{ux, x\}) \in \frK{\Q}$ contributes two 
ground queries for the set \groundings{\Q}: 
$$ 
{\setlength{\arraycolsep}{0em} 
\begin{array}{l} 
  \grounding{\Q_{fr}, \{ux, x\}, \{ux \mapsto a, x \mapsto b\}} = \\ 
  \{r(a, b), (\exists \inv{r}.\top)(a), (\exists r.((\exists (r \sqcap 
  \inv{s}).\top) \sqcap (\exists (t \sqcap \inv{t}).\top)))(b)\}, 
\end{array} 
} 
$$ 
where $\exists \inv{r}.\top$ is the query concept for the (tree-shaped) 
sub-query $\sq{\Q_{fr}, ux}$ and $\exists r.((\exists (r \sqcap 
\inv{s}).\top) \sqcap (\exists (t \sqcap \inv{t}).\top)$ is the query 
concept for $\sq{\Q_{fr}, x}$ and 
$$ 
{\setlength{\arraycolsep}{0.1em} 
\begin{array}{l} 
  \grounding{\Q_{fr}, \{ux, x\}, \{ux \mapsto b, x \mapsto a\}} = \\ 
  \{r(b, a), (\exists \inv{r}.\top)(b), (\exists r.((\exists (r \sqcap 
  \inv{s}).\top) \sqcap (\exists (t \sqcap \inv{t}).\top)))(a)\}. 
\end{array} 
} 
$$ 
The tuple $(\Q, \{u, x, y, z\}) \in \frK{\Q}$, however, does not 
contribute a ground query since, for a ground mapping, we require that 
$\tau(t) = \tau(t')$ iff $t \sapprox t'$ and there are only two 
individual names in \indA compared to four terms \Q that need a distinct 
value. Intuitively, this is not a restriction, since in the first 
rewriting step (collapsing) we produce all those queries in which the 
terms of \Q have been identified with each other in all possible ways. 
In our example, $\KB \models \Q$ and $\KB \models \Q_1 \vee \cdots \vee 
\Q_\ell$, where $\Q_1 \vee \cdots \vee \Q_\ell$ are the queries from 
\trees{\Q} and \groundings{\Q} since each model \I of \KB satisfies 
$\Q_i = \grounding{\Q_{fr}, \{ux, x\}, \{ux \mapsto a, x \mapsto b\}}$.


\subsection{Query Matches}
\label{sect:querymatches}

Even if a query is true in a canonical model, it does not necessarily 
mean that the query is tree- or forest-shaped. However, a match $\pi$ 
for a canonical interpretation can guide the process of rewriting a 
query. Similarly to the definition of tree- or forest-shaped queries, we 
define the shape of matches for a query. In particular, we introduce 
three different kinds of matches: \emph{split matches, forest matches}, 
and \emph{tree matches} such that every tree match is a forest match, 
and every forest match is a split match. The correspondence to the query 
shapes is as  follows: given a split match $\pi$, the set of all root 
nodes $(a, \varepsilon)$ in the range of the match define a root 
splitting for the query, if $\pi$ is additionally a forest match, the 
query is forest-shaped w.r.t.\ the root splitting induced by $\pi$, and 
if $\pi$ is additionally a tree match, then the whole query can be 
mapped to a single tree (i.e., the query is tree-shaped or forest-shaped 
w.r.t.\ an empty root splitting). Given an arbitrary query match into a 
canonical model, we can first obtain a split match and then a tree or 
forest match, by using the structure of the canonical model for guiding 
the application of the rewriting steps. 

\begin{definition}\label{def:matches}
  Let \KB be a \SHIQ knowledge base, \Q a query, \I = \inter a canonical 
  model of \KB, and $\pi \colon \terms{\Q} \to \dom$ an evaluation such 
  that $\I \models^\pi \Q$. We call $\pi$ a \emph{split match} if, for 
  all $r(t, t') \din \Q$, one of the following holds:
  \begin{enumerate}
    \item
      $\pi(t) = (a, \varepsilon)$ and $\pi(t') = (b, \varepsilon)$ for 
      some $a, b \in \indA$; or
    \item
      $\pi(t) = (a, w)$ and $\pi(t') = (a, w')$ for some $a \in \indA$ 
      and $w, w' \in \Nbbm^*$.
  \end{enumerate}
  We call $\pi$ a \emph{forest match} if, additionally, for each term 
  $t_r \in \terms{\Q}$ with $\pi(t_r) = (a, \varepsilon)$ and $a \in 
  \indA$, there is a total and bijective mapping $f$ from $\{(a, w) \mid 
  (a, w) \in \range{\pi}\}$ to a tree $T$ such that $r(t, t') \din 
  \sq{\Q, t_r}$ implies that $f(\pi(t))$ is a neighbor of $f(\pi(t'))$. 
%  
%  the following 
%  holds:
%  \begin{enumerate}
%    \item[2.]
%      \begin{enumerate}
%        \item[a)]
%          If $\pi(t) = (a, w)$ and $\pi(t') = (a, w')$ for some $a \in 
%          \indA$ and $w, w' \in \Nbbm^*$, then either $w$ is a proper 
%          prefix of $w'$ or $w'$ is a proper prefix of $w$ and, 
%        \item[b)]
%           for each $a \in \indA$, there is no pair of role atoms $r(t, 
%           t'), r'(t, t'') \din \Q$ with $\pi(t) = (a, w), \pi(t') = (a, 
%           w')$, and $\pi(t'') = (a, w'')$ and $w'$ is a proper prefix 
%           of $w''$.
%      \end{enumerate}
%  \end{enumerate}
  We call $\pi$ a \emph{tree match} if, additionally, there is an $a \in 
  \indA$ such that each element in $\range{\pi}$ is of the form $(a, 
  w)$.
  
  A split match $\pi$ for a canonical interpretation induces a (possibly 
  empty) root splitting \roots such that $t \in \roots$ iff $\pi(t) = 
  (a, \varepsilon)$ for some $a \in \indA$. We call \roots the 
  \emph{root splitting induced by $\pi$}. 
\end{definition}

For two elements $(a, w)$ and $(a, w')$ in a canonical model, the path 
from $(a, w)$ to $(a, w')$ is the sequence $(a, w_1), \ldots, (a, w_n)$ 
where $w = w_1, w' = w_n$, and, for $1 \leq i < n, w_{i+1}$ is a 
successor of $w_i$. The length of the path is $n$. Please note that, for 
a forest match, we do not require that $w$ is a neighbor of $w'$ or vice 
versa. This still allows to map role atoms to paths in the canonical 
model of length greater than two, but such paths must be between 
ancestors and not between elements in different branches of the tree. 
The mapping $f$ to a tree also makes sure that if \roots is the induced 
root splitting, then each sub-query \sq{\Q, t} for $t \in \roots$ is 
tree-shaped. For a tree match, the root splitting is either empty or $t 
\sapprox t'$ for each $t, t' \in \roots$, i.e., there is a single root 
modulo \sapprox, and the whole query is tree-shaped. 


\subsection{Correctness of the Query Rewriting}
\label{sect:correctnessrewriting}

The following lemmas state the correctness of the rewriting step by step 
for each of the rewriting stages. Full proofs are given in the 
appendix. As motivated in the previous section, we can use a given 
canonical model to guide the rewriting process such that we obtain a 
forest-shaped query that also has a match into the model. 

\begin{lemma}\label{lem:collapsing}
  Let \I be a model for \KB. 
  \begin{enumerate}
    \item\label{it:querycollapsing} 
      If $\I \models \Q$, then there is a collapsing $\Q_{co}$ of \Q 
      such that $\I \models^{\pi_{co}} \Q_{co}$ for $\pi_{co}$ an 
      injection modulo \sapprox. 
    \item\label{it:collapsingquery} 
      If $\I \models^{\pi_{co}} \Q_{co}$ for a collapsing $\Q_{co}$ of 
      \Q, then $\I \models \Q$.
  \end{enumerate}
\end{lemma}

Given a model \I that satisfies \Q, we can simply add equality atoms for 
all pairs of terms that are mapped to the same element in \I. It is not 
hard to see that this results in a mapping that is injective modulo 
\sapprox. For the second part, it is easy to see that a model that 
satisfies a collapsing also satisfies the original query.

\begin{lemma}\label{lem:splitrewriting}
  Let \I be a model for \KB. 
  \begin{enumerate}
    \item\label{it:one} 
      If \I is canonical and $\I \models^\pi \Q$, then there is a pair 
      $(\Q_{sr}, \roots) \in \srK{\Q}$ and a split match $\pi_{sr}$ such 
      that $\I \models^{\pi_{sr}} \Q_{sr}$, \roots is the induced root 
      splitting of $\pi_{sr}$, and $\pi_{sr}$ is an injection modulo 
      \sapprox.
    \item\label{it:two}
      If $(\Q_{sr}, \roots) \in \srK{\Q}$ and $\I \models^{\pi_{sr}} 
      \Q_{sr}$ for some match $\pi_{sr}$, then $\I \models \Q$.
  \end{enumerate}
\end{lemma}

For the first part of the lemma, we proceed exactly as illustrated in 
the example section and use the canonical model \I and the match $\pi$ 
to guide the rewriting steps. We first build a collapsing $\Q_{co} \in 
\co{\Q}$ as described in the proof of Lemma~\ref{lem:collapsing} such 
that $\I \models^{\pi_{co}} \Q_{co}$ for $\pi_{co}$ an injection modulo 
\sapprox. Since \I is canonical, paths between different trees can only 
occur due to non-simple roles, and thus we can replace each role atom 
that uses such a short-cut with two or three role atoms such that these 
roots are explicitly included in the query (cf.\ the query and match in 
Figure~\ref{fig:querymatch} and the obtained split rewriting and with a 
split match in Figure~\ref{fig:splitmatch}). The second part of the 
lemma follows immediately from the fact that we use only transitive 
sub-roles in the replacement.

\begin{lemma}\label{lem:looprewriting}
  Let \I be a model of \KB. 
  \begin{enumerate}
    \item
      If \I is canonical and $\I \models \Q$, then there is a pair 
      $(\Q_{\ell r}, \roots) \in \lrK{\Q}$ and a mapping $\pi_{\ell r}$ 
      such that $\I \models^{\pi_{\ell r}} \Q_{\ell r}$, $\pi_{\ell r}$ 
      is an injection modulo \sapprox, \roots is the root splitting 
      induced by $\pi_{\ell r}$ and, for each $r(t, t) \din \Q_{\ell 
      r}$, $t \in \roots$.
    \item 
      If $(\Q_{\ell r}, \roots) \in \lrK{\Q}$ and $\I 
      \models^{\pi_{\ell r}} \Q_{\ell r}$ for some match $\pi_{\ell r}$, 
      then $\I \models \Q$.
  \end{enumerate}
\end{lemma}

The second part is again straightforward, given that we can only use 
transitive sub-roles in the loop rewriting. For the first part, we 
proceed again as described in the examples section and use the canonical 
model \I and the match $\pi$ to guide the rewriting process. We first 
build a split rewriting $\Q_{sr}$ and its root splitting \roots as 
described in the proof of Lemma~\ref{lem:splitrewriting} such that 
$(\Q_{sr}, \roots) \in \srK{\Q}$ and $\I \models^{\pi_{sr}} \Q_{sr}$ for 
a split match $\pi_{sr}$. Since \I is a canonical model, it has a forest 
base \Jmc. In a forest base, non-root nodes cannot be successors of 
themselves, so each such loop is a short-cut due to some transitive 
role. An element that is, say, $r$-related to itself has, therefore, a 
neighbor that is both an $r$- and $\inv{r}$-successor. Depending on 
whether this neighbor is already in the range of the match, we can 
either re-use an existing variable or introduce a new one, when making 
this path explicit (cf.\ the loop rewriting depicted in 
Figure~\ref{fig:looprewriting} obtained from the split rewriting shown 
in Figure~\ref{fig:splitmatch}). 

\begin{lemma}\label{lem:forestrewriting}
  Let \I be a model of \KB. 
  \begin{enumerate}
    \item
      If \I is canonical and $\I \models \Q$, then there is a pair 
      $(\Q_{fr}, \roots) \in \frK{\Q}$ such that $\I \models^{\pi_{fr}} 
      \Q_{fr}$ for a forest match $\pi_{fr}$, \roots is the induced root 
      splitting of $\pi_{fr}$, and $\pi_{fr}$ is an injection modulo 
      \sapprox.
    \item 
      If $(\Q_{fr}, \roots) \in \frK{\Q}$ and $\I \models^{\pi_{fr}} 
      \Q_{fr}$ for some match $\pi_{fr}$, then $\I \models \Q$.
  \end{enumerate}
\end{lemma}

The main challenge is again the proof of (1) and we just give a short 
idea of it here. At this point, we know from 
Lemma~\ref{lem:looprewriting} that we can use a query $\Q_{\ell r}$ for 
which there is a root splitting \roots and a split match $\pi_{\ell r}$. 
Since $\pi_{\ell r}$ is a split match, the match for each such sub-query 
is restricted to a tree and thus we can transform each sub-query of 
$\Q_{\ell r}$ induced by a term $t$ in the root choice separately. The 
following example is meant to illustrate why the given bound of 
$\card{\vars{\Q}}$ on the number of new variables and role atoms that 
can be introduced in a forest rewriting suffices. 
Figure~\ref{fig:treeification1} depicts the representation of a tree 
from a canonical model, where we use only the second part of the names 
for the elements, e.g., we use just $\varepsilon$ instead of $(a, 
\varepsilon)$. For simplicity, we also do not indicate the concepts and 
roles that label the nodes and edges, respectively. We use black color 
to indicate the nodes and edges that are used in the match for a query 
and dashed lines for short-cuts due to transitive roles. In the example, 
the grey edges are also those that belong to the forest base and the 
query match uses only short-cuts.

\begin{figure}[htb]
  \centering
  \input{treeification1.pstex_t}
  \caption{A part of a representation of a canonical model, where the 
  black nodes and edges are used in a match for a query and dashed edges 
  indicate short-cuts due to transitive roles.}
  \label{fig:treeification1}
\end{figure}

The forest rewriting aims at making the short-cuts more explicit by 
replacing them with as few edges as necessary to obtain a tree match. In 
order to do this, we need to include the ``common ancestors'' in the 
forest base between each two nodes used in the match. For $w, w' \in 
\Nbbm^*$, we therefore define the \emph{longest common prefix} (LCP) of 
$w$ and $w'$ as the longest $\hat{w} \in \Nbbm^*$ such that $\hat{w}$ is 
a prefix of both $w$ and $w'$. For a forest rewriting, we now determine 
the LCPs of any two nodes in the range of the match and add a variable 
for those LCPs that are not yet in the range of the match to the set $V$ 
of new variables used in the forest rewriting. In the example from 
Figure~\ref{fig:treeification1} the set $V$ contains a single variable 
$v_1$ for the node $1$. 

We now explicate the short-cuts as follows: for any edge used in the 
match, e.g., the edge from $\varepsilon$ to $111$ in the example, we 
define its \emph{path} as the sequence of elements on the path in the 
forest base, e.g., the path for the edge from $\varepsilon$ to $111$ is 
$\varepsilon, 1, 11, 111$. The \emph{relevant path} is obtained by 
dropping all elements from the path that are not in the range of the 
mapping or correspond to a variable in the set $V$, resulting in a 
relevant path of $\varepsilon, 1, 111$ for the example. We now replace 
the role atom that was matched to the edge from $\varepsilon$ to $111$ 
with two role atoms such that the match uses the edge from $\varepsilon$ 
to $1$ and from $1$ to $111$. An appropriate transitive sub-role exists 
since otherwise there could not be a short-cut. Similar arguments can be 
used to replace the role atom mapped to the edge from $111$ to $12$ and 
for the one that is mapped to the edge from $\varepsilon$ to $12$, 
resulting in a match as represented by Figure~\ref{fig:treeification2}. 
The given restriction on the cardinality of the set $V$ is no limitation 
since the number of LCPs in the set $V$ is maximal if there is no pair 
of nodes such that one is an ancestor of the other. We can see these 
nodes as $n$ leaf nodes of a tree that is at least binarily branching. 
Since such a tree can have at most $n$ inner nodes, we need at most $n$ 
new variables for a query in $n$ variables. 

\begin{figure}[htb]
  \centering
  \input{treeification2.pstex_t}
  \caption{The match for a forest rewriting obtained from the example 
  given in Figure~\ref{fig:treeification1}.}
  \label{fig:treeification2}
\end{figure}

For the bound on the number of role atoms that can be used in the 
replacement of a single role atom, consider, for example, the cyclic 
query 
$$
\Q = \{r(x_1, x_2), r(x_2, x_3), r(x_3, x_4), t(x_1, x_4)\}, 
$$
for the knowledge base \KBDef with $\TB = \emptyset, \RB = \{r 
\sqsubseteq t\}$ with $t \in \transR$ and $\AB = \{(\exists r.(\exists 
r.(\exists r.\top)))(a)\}$. It is not hard to check that $\KB \models 
\Q$. Similarly to our running example from the previous section, there 
is also a single rewriting that is true in each canonical model of the 
KB, which is obtained by building only a forest rewriting and doing 
nothing in the other rewriting steps, except for choosing the empty set 
as root splitting in the split rewriting step. In the forest rewriting, 
we can explicate the short-cut used in the mapping for $t(x_1, x_4)$ by 
replacing $t(x_1, x_4)$ with $t(x_1, x_2), t(x_2, x_3), t(x_3, x_4)$. 

By using Lemmas~\ref{lem:collapsing} to \ref{lem:forestrewriting}, we 
get the following theorem, which shows that we can use the ground 
queries in \groundings{\Q} and the queries in \trees{\Q} in order to 
check whether \KB entails \Q, which is a well understood problem. 

\begin{theorem}\label{thm:union} 
  Let \KB be a \SHIQ knowledge base, \Q a Boolean conjunctive query, and 
  $\{\Q_1, \ldots, \Q_\ell\} = \trees{\Q} \cup \groundings{\Q}$. Then 
  $\KB \models \Q$ iff $\KB \models \Q_1 \vee \ldots \vee \Q_\ell$.
\end{theorem}

We now give upper bounds on the size and number of queries in \trees{\Q} 
and \groundings{\Q}. As before, we use $\card{S}$ to denote the 
\emph{cardinality} of a set $S$. The \emph{size} $|\KB|$ ($|\Q|$) of a 
knowledge base \KB (a query \Q) is simply the number of symbols needed 
to write it over the alphabet of constructors, concept names, and role 
names that occur in \KB (\Q), where numbers are encoded in binary. 
Obviously, the number of atoms in a query is bounded by its size, hence 
$\card{\Q} \leq |\Q|$ and, for simplicity, we use $n$ as the size 
and the cardinality of \Q in what follows. 

\begin{lemma}\label{lem:counting}
  Let \Q be a Boolean conjunctive query, \KBDef a \SHIQ knowledge base, 
  $|\Q| := n$ and $|\KB| := m$. Then there is a polynomial $p$ such that
  \begin{enumerate}
    \item\label{it:co} 
      $\card{\co{\Q}} \leq 2^{p(n)}$ and, for each $\Q' \in 
      \co{\Q}$, $|\Q'| \leq p(n)$, 
    \item\label{it:sr}
      $\card{\srK{\Q}} \leq 2^{p(n) \cdot \log p(m)}$, and, for 
      each $\Q' \in \srK{\Q}$, $|\Q'| \leq p(n)$, 
    \item\label{it:lr}
      $\card{\lrK{\Q}} \leq 2^{p(n) \cdot \log p(m)}$, and, for 
      each $\Q' \in \lrK{\Q}$, $|\Q'| \leq p(n)$, 
    \item\label{it:fr}
      $\card{\frK{\Q}} \leq 2^{p(n) \cdot \log p(m)}$, and, for 
      each $\Q' \in \frK{\Q}$, $|\Q'| \leq p(n)$, 
    \item\label{it:trees} 
      $\card{\trees{\Q}} \leq 2^{p(n) \cdot \log p(m)}$, and, for 
      each $\Q' \in \trees{\Q}$, $|\Q'| \leq p(n)$, and 
    \item\label{it:groundings} 
      $\card{\groundings{\Q}} \leq 2^{p(n) \cdot \log p(m)}$, and, 
      for each $\Q' \in \groundings{\Q}$, $|\Q'| \leq p(n)$.
  \end{enumerate}
\end{lemma}

As a consequence of the above lemma, there is a bound on the number of 
queries in \groundings{\Q} and \trees{\Q} and it is not hard to see that 
the two sets can be computed in time polynomial in $m$ and exponential 
in $n$. 

In the next section, we present an algorithm that decides entailment of 
unions of conjunctive queries, where each of the queries is either a 
ground query or consists of a single concept atom $C(x)$ for an 
existentially quantified variable $x$. By Theorem~\ref{thm:union} and 
Lemma~\ref{lem:counting}, such an algorithm is a decision procedure for 
arbitrary unions of conjunctive queries. 



\subsection{Summary and Discussion}

In this section, we have presented the main technical foundations for 
answering (unions of) conjunctive queries. It is known that queries that 
contain non-simple roles in cycles among existentially quantified 
variables are difficult to handle. By applying the rewriting steps from 
Definition~\ref{def:rewriting}, we can rewrite such cyclic conjunctive 
queries into a set of acyclic and/or ground queries. Both types of 
queries are easier to handle and algorithms for both types exist. At 
this point, any reasoning algorithm for \SHIQR knowledge base 
consistency can be used for deciding query entailment. In order to 
obtain tight complexity results, we present in the following section a 
decision procedure that is based on an extension of the translation to 
looping tree automata given by \citeA{Tobi01a}. 

It is worth mentioning that, for queries with only simple roles, our 
algorithm behaves exactly as the existing rewriting algorithms (i.e., 
the rolling-up and tuple graph technique) since, in this case, only the 
collapsing step is applicable. The need for identifying variables was 
first pointed out in the work of \citeA{HSTT99a} and is also required 
(although not mentioned) for the algorithm proposed by \citeA{CaDL98a}. 

The new rewriting steps (split, loop, and forest rewriting) are only 
required for and applicable to non-simple roles and, when replacing a 
role atom, only transitive sub-roles of the replaced role can be used. 
Hence the number of resulting queries is in fact not determined by the 
size of the whole knowledge base, but by the number of transitive 
sub-roles for the non-simple roles in the query. Therefore, the number 
of resulting queries really depends on the number of transitive roles 
and the depth of the role hierarchy for the non-simple roles in the 
query, which can, usually, expected to be small. 
